On Synergistic Benefits of Rate Splitting in IRS-assisted Cloud Radio Access Networks

The concept of intelligent reflecting surfaces (IRSs) is considered as a promising technology for increasing the efficiency of mobile wireless networks. This is achieved by employing a vast amount of low-cost individually adjustable passive reflect elements, that are able to apply changes to the reflected signal. To this end, the IRS makes the environment realtime controllable and can be adjusted to significantly increase the received signal quality at the users by passive beamsteering. However, the changes to the reflected signals have an effect on all users near the IRS, which makes it impossible to optimize the changes to positively influence every transmission, affected by the reflections. This results in some users not only experiencing better signal quality, but also an increase in received interference. To mitigate this negative side effect of the IRS, this paper utilizes the rate splitting (RS) technique, which enables the mitigation of interference within the network in such a way that it also mitigates the increased interference caused by the IRS. To investigate the effects on the overall power savings, that can be achieved by combining both techniques, we minimize the required transmit power, needed to satisfy per-user quality-of-service (QoS) constraints. Numerical results show the improved power savings, that can be gained by utilizing the IRS and the RS technique simultaneously. In fact, the concurrent use of both techniques yields power savings, which are beyond the cumulative power savings of using each technique separately.

==> Publish5 v9 (conference-arxiv)/abstract.tex <==
\begin{abstract}
%\thispagestyle{plain}
The concept of \acp{IRS} is considered as a promising technology for increasing the efficiency of mobile wireless networks. This is achieved by employing a vast amount of low-cost individually adjustable passive reflect elements, that are able to apply changes to the reflected signal. To this end, the \ac{IRS} makes the environment real-time controllable and can be adjusted to significantly increase the received signal quality at the users by passive beamsteering. However, the changes to the reflected signals have an effect on all users near the \ac{IRS}, which makes it impossible to optimize the changes to positively influence every transmission, affected by the reflections. This results in some users not only experiencing better signal quality, but also an increase in received interference. To mitigate this negative side effect of the \ac{IRS}, this paper utilizes the \ac{RS} technique, which enables the mitigation of interference within the network in such a way that it also mitigates the increased interference caused by the \ac{IRS}. To investigate the effects on the overall power savings, that can be achieved by combining both techniques, we minimize the required transmit power, needed to satisfy per-user \ac{QoS} constraints. Numerical results show the improved power savings, that can be gained by utilizing the \ac{IRS} and the \ac{RS} technique simultaneously. In fact, the concurrent use of both techniques yields power savings, which are beyond the cumulative power savings of using each technique separately.
\end{abstract} 

==> Publish5 v9 (conference-arxiv)/commands/commands.tex <==
\newcommand{\blank}[1]{\hfil\penalty1000\hfilneg\rule[-3pt]{#1}{0.4pt}} % nice blank underscores
\newcommand{\modernBS}{
	\begin{tikzpicture}[scale=.6]
	{
		\draw (0,1) -- (0,-0.8) node [pos=0.3]  (middletop){};
		\draw (0,1) -- (0,-0.8) node [pos=0.75] (middlebot){};
		\draw (0,1) -- (0.5,-0.5) node [pos=0.3] (righttop){};
		\draw (0,1) -- (0.5,-0.5) node [pos=0.75](rightbot){};
		\draw (0,1) -- (-0.5,-0.5)node [pos=0.3] (lefttop){};
		\draw (0,1) -- (-0.5,-0.5)node [pos=0.75](leftbot){};
		\draw (-0.5,-0.5) -- (0,-0.8) -- (0.5,-0.5);
		\draw (righttop.center)-- (middletop.center) -- (lefttop.center);
		\draw (rightbot.center)-- (middlebot.center) -- (leftbot.center);
	}
	\end{tikzpicture}	
}

\newcommand{\modernBuildingWindow}{
   \begin{tikzpicture}
%      \node[rectangle,draw,minimum width=] at (0,0){};
   \end{tikzpicture}
}

\newcommand{\modernBuilding}{
	\begin{tikzpicture}[scale=2]
	{
		\draw (0,1) -- (0,-0.8) node [pos=0.9]  (middletop){};
		\draw (0.5,1.3) -- (0.5,-0.5) node [pos=0.9] (righttop){};
      \draw (-0.5,1.3) -- (-0.5,-0.5)node [pos=0.9] (lefttop){};

      \foreach \pos in {0.8,0.7,...,0}
      {
      \path (0,1) -- (0,-0.8) node [pos=\pos] (middlebot){};
      \path (0.5,1.3) -- (0.5,-0.5) node [pos=\pos] (rightbot){};
      \path (-0.5,1.3) -- (-0.5,-0.5)node [pos=\pos] (leftbot){};

%
%      \draw (righttop.center)-- (middletop.center) -- (lefttop.center);
%
%      \draw (rightmid.center)-- (middlemid.center) -- (leftmid.center);
		\draw[line width=0.2] (rightbot.center)-- (middlebot.center) -- (leftbot.center);
   }
    \foreach \pos in {0.75,0.5,...,0}
    {
		\draw (0.5,1.3) -- (0,1) node [pos=\pos] (w1-1){};
      \path (0.5,1.3) -- (0,1) node [pos=\pos]{};
      \draw (0.5,-0.5)--(0,-0.8) node [pos=\pos](w1-2){};

      \draw[line width=0.1] (w1-1.center) -- (w1-2.center);
    }
      \draw (-0.5,1.3) -- (0,1);
		\draw (-0.5,-0.5) -- (0,-0.8);
     \foreach \pos in {0.75,0.5,...,0}
    {
		\path (-0.5,1.3) -- (0,1)node [pos=\pos](x1){};
		\path (-0.5,-0.5) -- (0,-0.8) node [pos=\pos](x2){};
      \draw[line width=0.1] (x1.center)--(x2.center);
     }
      \draw (0.5,-0.5)--(0,-0.8) node [pos=0.75](w1-2){};
      \draw (0,1.6) -- (-0.5,1.3) node [pos=0.75]{};
      \draw (0,1.6) -- (0.5,1.3) node [pos=0.75]{};


%		\path (0,1) -- (0,-0.8) node [pos=0.6]  (middletop){};
%		\path (0,1) -- (0,-0.8) node [pos=0.9] (middlebot){};
%      \path (0,1) -- (0,-0.8) node [pos=0.45] (middlemid){};
%		\path (0.5,1.3) -- (0.5,-0.5) node [pos=0.7] (righttop){};
%      \path (0.5,1.3) -- (0.5,-0.5) node [pos=0.9] (rightbot){};
%      \path (0.5,1.3) -- (0.5,-0.5) node [pos=0.45] (rightmid){};
%      \path (-0.5,1.3) -- (-0.5,-0.5)node [pos=0.6] (lefttop){};
%		\path (-0.5,1.3) -- (-0.5,-0.5)node [pos=0.9] (leftbot){};
%      \path (-0.5,1.3) -- (-0.5,-0.5)node [pos=0.45] (leftmid){};
%
%		\draw (righttop.center)-- (middletop.center) -- (lefttop.center);
%%      \draw (rightmid.center)-- (middlemid.center) -- (leftmid.center);
%		\draw (rightbot.center)-- (middlebot.center) -- (leftbot.center);

	}
      \path (-0.5,-0.5) -- (0,-0.8) node [pos=0.5](door1){};
      \node[yslant=-0.6,rectangle,draw] at ($(door1)+(0,0.075)$){};
      \node[yslant=-0.6,circle,draw,scale=0.1,line width=0.2] at ($(door1)+(0.02,0.055)$){};
      \node[yslant=-0.6,circle,draw,scale=0.1,line width=0.2] at ($(door1)+(-0.02,0.075)$){};
	\end{tikzpicture}	
}

\newcommand{\skewedIRS}{
	\begin{tikzpicture}
		\node[rectangle,minimum width=1.5cm,minimum height=1.5cm,draw,yslant=-0.6,scale=0.5,fill=blue!20!green] at (0,0){};

		\node[rectangle,minimum width=0.05cm,minimum height=0.05cm,draw,yslant=-0.6,scale=0.25,fill=yellow!70!green] (base) at (-0.3,-0.12){};

         \foreach \y in {1,...,5}
         {
            \node[rectangle,minimum width=0.05cm,minimum height=0.05cm,draw,yslant=-0.6,scale=0.25,fill=yellow!70!green] at
            ($($(base)+(-31:0.14*0)$)+(90:0.12*\y)$){};
         }

      \foreach \x in {1,...,5}
      {
         \node[rectangle,minimum width=0.05cm,minimum height=0.05cm,draw,yslant=-0.6,scale=0.25,fill=yellow!70!green] at
         ($(base)+(-31:0.14*\x)$){};

         \foreach \y in {1,...,5}
         {
            \node[rectangle,minimum width=0.05cm,minimum height=0.05cm,draw,yslant=-0.6,scale=0.25,fill=yellow!70!green] at
            ($($(base)+(-31:0.14*\x)$)+(90:0.12*\y)$){};
         }
      }
	\end{tikzpicture}	
}
\tikzset{hexagon/.code={
	\draw (0,2) -- (-4,0) -- (0,-2) -- (4,0) -- (0,2);
}}

\tikzset{phone/.code={
   \node [rectangle,rounded corners=1.5pt,draw,minimum height=0.6cm, minimum width=0.35cm] at (0,0){};
   \node [rectangle,rounded corners=1.5pt,draw,minimum height=0.5cm, minimum width=0.3cm] at (0,0){};
}}

\newcommand\hcancel[2][black]{\setbox0=\hbox{$#2$}%
\rlap{\raisebox{.45\ht0}{\textcolor{#1}{\rule{\wd0}{1pt}}}}#2}
\makeatletter
% #1, #2 offset of label   #6 extra width to clear arrowhead
% #3, #4 vector direction  #7 superscript label style
% #5 vector width          #8 superscript label
\def\cantox@vector#1#2#3#4#5#6#7#8{%
  \dimen@.5\p@
  \setbox\z@\vbox{\boxmaxdepth.5\p@
   \hbox{\kern-1.2\p@\kern#1\dimen@$#7{#8}\m@th$}}%
  \ifx\canto@fil\hidewidth  \wd\z@\z@ \else \kern-#6\unitlength \fi
  \ooalign{%
    \canto@fil$\m@th \CancelColor
    \vcenter{\hbox{\dimen@#6\unitlength \kern\dimen@
      \multiply\dimen@#4\divide\dimen@#3 \vrule\@depth\dimen@\@width\z@
      \vector(#3,-#4){#5}%
    }}_{\raise-#2\dimen@\copy\z@\kern-\scriptspace}$%
    \canto@fil \cr
    \hfil \box\@tempboxa \kern\wd\z@ \hfil \cr}}
\def\bcancelto#1#2{\let\canto@vector\cantox@vector\cancelto{#1}{#2}}
\makeatother

\newcommand{\ifthen}[2]{\ifthenelse{#1}{#2}{}}
\newcommand{\colorRed}[1]{\textcolor{red}{#1}}
\newcommand{\myNorm}[1]{\left\lVert#1\right\rVert}
\newcommand{\trNorm}[1]{\left\lVert#1\right\rVert_{\text{Tr}}}
\newcommand{\tildeV}{\tilde{\vect{v}}}
\newcommand{\sqr}[1]{{#1}^2}
\newcommand{\sbrackets}[1]{\left(#1\right)}
\newcommand{\hbrackets}[1]{\left[#1\right]}
\newcommand{\vectw}{\vect{\omega}}
\newcommand{\vectv}{\vect{v}}
\newcommand{\vectvt}{\tilde{\vect{v}}}
\newcommand{\matV}{\mat{V}}
\newcommand{\matX}{\mat{X}}
\newcommand{\vecth}{\vect{h}}
\newcommand{\matH}{\mat{H}}
\newcommand{\vecta}{\vect{a}}
\newcommand{\matM}{\mat{M}}
\newcommand{\matOmega}{\mat{W}}
\newcommand{\vectTheta}{\mat{\theta}}
\newcommand{\cbrackets}[1]{\left\{#1\right\}}
\newcommand{\Tr}[1]{\text{Tr}\left(#1\right)}
\renewcommand{\rank}[1]{\text{rank}\left(#1\right)}

\def\phone{{\tikz\node[phone]{};}}


\newcommand{\IRS}{
	\begin{tikzpicture}
		\node[rectangle,minimum width=1.5cm,minimum height=1.5cm,draw,scale=0.5,fill=blue!20!green] at (0,0){};

		\node[rectangle,minimum width=0.05cm,minimum height=0.05cm,draw,scale=0.25,fill=yellow!70!green] (base) at (-0.3,-0.3){};

         \foreach \y in {1,...,5}
         {
            \node[rectangle,minimum width=0.05cm,minimum height=0.05cm,draw,scale=0.25,fill=yellow!70!green] at
            ($($(base)+(-31:0.14*0)$)+(90:0.12*\y)$){};
         }

      \foreach \x in {1,...,5}
      {
         \node[rectangle,minimum width=0.05cm,minimum height=0.05cm,draw,scale=0.25,fill=yellow!70!green] at
         ($(base)+(0:0.12*\x)$){};

         \foreach \y in {1,...,5}
         {
            \node[rectangle,minimum width=0.05cm,minimum height=0.05cm,draw,scale=0.25,fill=yellow!70!green] at
            ($($(base)+(0:0.12*\x)$)+(90:0.12*\y)$){};
         }
      }
	\end{tikzpicture}	
}


%% needed for "List of Equations"
\newcommand{\listequationsname}{List of Formulas}
\newlistof{myequations}{equ}{\listequationsname}
\newcommand{\myequations}[1]{%
\addcontentsline{equ}{myequations}{\protect\numberline{\theequation}#1}\par
}


%% own colors
\definecolor{myblue1}{rgb}{0,0,255}
\definecolor{myblue2}{rgb}{65,105,225}
\definecolor{myblue3}{rgb}{70,130,180}
\definecolor{myblue4}{rgb}{176,196,222}



%% own commands
\newcommand{\mytilde}{{\raise.17ex\hbox{$\scriptstyle\mathtt{\sim}$}}}
\newcommand{\naive}{}
\def\naive/{na\"{\i}ve}
\newcommand{\changefont[3]}{\fontfamily{#1}\fontseries{#2}\fontshape{#3}\selectfont}
\newcommand{\executeiffilenewer}[3]{%
\ifnum\pdfstrcmp{\pdffilemoddate{#1}}%
{\pdffilemoddate{#2}}>0%
{\immediate\write18{#3}}\fi%
}
% includesvg[scale]{file} command (linux-version)
\newcommand{\includesvg}[2][1]{%
  \executeiffilenewer{#1.svg}{#1.pdf}{%
  /usr/bin/inkscape -z -D --file="#2.svg" --export-pdf="#2.pdf" --export-latex}%
  \scalebox{#1}{\input{#2.pdf_tex}}%
}


% mobile phone
%\input{images/ber-plot}
\newcommand{\incmyber}[3]{% args: label, scale, position
\node (#1) at (#2) {\scalebox{#3}{\myber}};
}

\renewcommand*{\mod}{\,\mathrm{mod}\,}
\renewcommand*{\gcd}{\mathrm{gcd}}

\newcommand{\E}{\mathrm{E}}
\newcommand{\myY}{\mathbf{Y}}
\newcommand{\myX}{\mathbf{X}}
\newcommand{\myC}{\mathbf{C}}
\newcommand{\myA}{\mathbf{A}}
\newcommand{\myI}{\mathbf{I}}

%\pgfmathdeclarefunction{gauss}{2}{%
%  \pgfmathparse{1/(#2*sqrt(2*pi))*exp(-((x-#1)^2)/(2*#2^2))}%
%  }


\newcommand{\mysum}[2]{% args: label, pos
\node (#1) at (#2) [draw, thick, fill=white, drop shadow, circle, inner sep=3mm, scale=0.65] {};
\draw[thick] (#1.north) to (#1.south);
\draw[thick] (#1.west) to (#1.east);
}

\newcommand{\mysplit}[2]{% args: label, pos
\node (#1) [dot] at (#2) {};
}



\newcommand{\mybit}{[\mathrm{Bit}]}

\pgfkeys{/pgf/fpu}
\pgfmathparse{16383+1}
\edef\tmp{\pgfmathresult}
\pgfkeys{/pgf/fpu=false}


==> Publish5 v9 (conference-arxiv)/content/acronyms.tex <==
%\section{Acronyms}
\begin{acronym}
\setlength{\itemsep}{0.1em}
\acro{AF}{amplify-and-forward}
\acro{AWGN}{additive white Gaussian noise}
\acro{B5G}{Beyond 5G}
\acro{BS}{base station}
\acro{C-RAN}{Cloud Radio Access Network}
\acro{CMD}{common message decoding}
\acro{CP}{central processor}
\acro{D2D}{device-to-device}
\acro{DC}{difference-of-convex}
\acro{IC}{interference channel}
\acro{i.i.d.}{independent and identically distributed}
\acro{IRS}{intelligent reflecting surface}
\acro{IoT}{Internet of Things}
\acro{LoS}{line-of-sight}
\acro{M2M}{Machine to Machine}
\acro{MIMO}{multiple-input and multiple-output}
\acro{MRC}{maximum ratio combining}
\acro{NLoS}{non-line-of-sight}
\acro{PSD}{positive semidefinite}
\acro{QCQP}{quadratically constrained quadratic programming}
\acro{QoS}{quality-of-service}
\acro{RF}{radio frequency}
\acro{RS-CMD}{rate splitting and common message decoding}
\acro{RS}{rate splitting}
\acro{SDP}{semidefinite programming}
\acro{SDR}{semidefinite relaxation}
\acro{SIC}{Successive Interference Cancellation}
\acro{SINR}{signal-to-interference-plus-noise ratio}
\acro{SOCP}{second-order cone program}
\acro{SVD}{singular value decomposition }
\acro{TIN}{treating interference as noise}
\acro{UHDV}{Ultra High Definition Video}

%\acro{M2M}{Machine to Machine}
%\acro{B5G}{Beyond 5G}
%\acro{CP}{Central Processor}
%\acro{IRS}{Intelligent Reflecting Surface}
%\acro{IoT}{Internet of Things}
%\acro{BS}{base station}
%\acro{C-RAN}{Cloud Radio Access Network}
%\acro{TIN}{treating interference as noise}
%\acro{RS}{rate splitting}
%\acro{CMD}{common message decoding}
%\acro{RS-CMD}{rate splitting and common message decoding}
%\acro{UHDV}{Ultra High Definition Video}
%\acro{LoS}{line-of-sight}
%\acro{NLoS}{non-line-of-sight}
%\acro{AF}{amplify-and-forward}
%\acro{RF}{radio frequency}
%\acro{QoS}{quality-of-service}
%\acro{QCQP}{quadratically constrained quadratic programming}
%\acro{DC}{difference-of-convex}
%\acro{IC}{interference channel}
%\acro{SIC}{Successive Interference Cancellation}
%\acro{AWGN}{Additive White Gaussian Noise}
%\acro{SINR}{signal-to-interference-plus-noise
%ratio}
%\acro{SINRs}{signal-to-interference-plus-noise
%ratios}
%\acro{MRC}{maximum ratio combining}
%\acro{D2D}{device-to-device}
%\acro{MIMO}{multiple-input and multiple-output}
%\acro{i.i.d.}{independent and identically distributed}
%\acro{SOCP}{second-order cone program}
%\acro{SDR}{semidefinite relaxation}
%\acro{SDP}{semidefinite programming}
%\acro{PSD}{positive semidefinite}
%\acro{SVD}{singular value decomposition}
\end{acronym}


==> Publish5 v9 (conference-arxiv)/sections/alternatingMinimization.tex <==
\input{sections/alternatingMinimization/w_problem.tex}
\input{sections/alternatingMinimization/v_problem.tex}
\input{sections/alternatingMinimization/obtaining_optimal_solution.tex}



==> Publish5 v9 (conference-arxiv)/sections/alternatingMinimization/obtaining_optimal_solution.tex <==
The proposed alternating optimization algorithm for solving problem (\ref{eq:genProb}) is outlined in Algorithm \ref{alg:final}, where problems (\ref{eq:genW}) and (\ref{eq:genV-alpha_rank}) are solved alternatively.
\begin{algorithm}
\footnotesize
\caption{Procedure to determine $\vectw^*$ and $\vectv^*$ of (\ref{eq:genProb})}\label{alg:final}
\begin{algorithmic}
\STATE \textbf{Input: } $\vectv_0$, $z\leftarrow0$,  threshold $\epsilon$, number of Gaussian randomizations $G$
\STATE Initialize: Find feasible $\widehat{\mat{\Lambda}}_0 = \hbrackets{({\vect{w}_0)}^T ,\,({\vect{t}_0)}^T  }^T$
\WHILE{the decrease of $P^{\text{Tr}}(\vect{\omega})$ is below $\epsilon$}  \IF{problem (\ref{eq:genV-alpha_rank}) is feasible}
   \IF{at least one feasible candidate $\overline{\vectv}_g$ can be determined}
      \STATE Set $\tilde{\mat{\Lambda}} \leftarrow \widehat{\mat{\Lambda}}_z$
      \STATE Obtain $\widehat{\mat{\Lambda}}_{z+1}$ by solving problem (\ref{eq:cmpW})
      \STATE Obtain $\vectv_{z+1}$ by solving problem (\ref{eq:genV-alpha_rank})
      \STATE $z \leftarrow z+1$
   \ENDIF
\ENDIF
\ENDWHILE
\STATE$\vectw^* \leftarrow \vectw_z$, $\vectv^* \leftarrow \vectv_z$
\STATE \textbf{Output: } Optimal $\vectw^*$ and optimal $\vectv^*$.
\end{algorithmic}
\end{algorithm} 



==> Publish5 v9 (conference-arxiv)/sections/alternatingMinimization/v_problem.tex <==
\subsection{Phase Shift Design}
Given $\mat{\Lambda} = \hbrackets{\vect{w}^T ,\,\vect{t}^T}^T$, which is assumed to be fixed for the duration of optimizing the phase shift vector $\vectv$, Problem (\ref{eq:genProb}) can be expressed as a \ac{QCQP} problem {\cite{IRSImprovement1}. To this end, problem (\ref{eq:genProb}) can be reformulated into
\begin{align}\label{eq:genV-reform1}
   \text{find}\qquad &  \vect{v} \tag{P3.1}\\
   \text{subject to} \qquad
    &\gamma_k^p(\vectv) \geq t_k^p, && \forall k \in \mathcal{K} \label{eq:reform1_v-p}\\
    &\gamma_{i,k}^c(\vectv)\geq t_k^c,  && \forall k \in \mathcal{K} ,\, \forall i \in \mathcal{M}_k \label{eq:reform1_v-c}\\
    & | v_r | = 1,  && \forall r \in \{ 1,..., R\},
\end{align}
where the constraints (\ref{eq:reform1_v-p}) and (\ref{eq:reform1_v-c}) can be rewritten as
\begin{align}\label{eq:genV-reform2-p}
        &\hspace{-0.25cm}|\left( \vect{h}_k + \mat{H}_k \vect{v} \right)^H \vect{\omega}_k^p|^2 \geq t_k^p \left(
        \sum_{j\in\mathcal{K}\text{\textbackslash}\cbrackets{k}} \hspace{-0.175cm}|\left( \vect{h}_k + \mat{H}_k \vect{v} \right)^H \vect{\omega}_j^p|^2+ \right.\nonumber \\
        & \left.  \sum_{\ell \in \Psi_k} |\left( \vect{h}_k + \mat{H}_k \vect{v} \right)^H \vect{\omega}_\ell^c|^2 + \sigma^2\right), \hspace{1cm} \forall k \in \mathcal{K}
        \end{align}
        \begin{align}
         &\hspace{-0.2cm}|\left( \vect{h}_i + \mat{H}_i \vect{v} \right)^H \vect{\omega}_k^c|^2 \geq t_k^c\sbrackets{
         T_i + \sum_{\ell \in \Psi_i} |\left( \vect{h}_i + \mat{H}_i \vect{v} \right)^H \vect{\omega}_\ell^c|^2+ \right. \nonumber \\
         & \hspace{0.25cm} \left. \hspace{-0.2cm} \sum_{m \in \Omega_{i,k}} \hspace{-0.25cm} |\left( \vect{h}_i + \mat{H}_i \vect{v} \right)^H \vect{\omega}_m^c|^2},\forall k \in \mathcal{K} ,\, \forall i \in \mathcal{M}_k.\label{eq:genV-reform2-c}
\end{align}
This facilitates denoting
\begin{align}
   b_{k,i}^o &= \vect{h}_k^H \vectw_i^o, \text{ and }
   \vecta_{k,i}^o = \matH_k^H \vectw_i^o, \\
   \mat{M}_{k,j}^o &=
         \begin{bmatrix}
            \vect{a}_{k,j}^o ({\vect{a}_{k,j}^o})^H & \vect{a}_{k,j}^o (b_{k,j}^o)^H  \\
            {b_{k,j}^o} ({\vect{a}_{k,j}^o})^H  & 0  \\
         \end{bmatrix} \\
        \tilde{\vect{v}} \,&= \,[\vect{v}^T, s]^T,\label{eq:auxVar}
\end{align}
where $s$ is an auxiliary variable. Due to the auxiliary variable $s$, it holds that if a feasible solution $\vectvt^*$ is found, a solution $\vect{v}^*$ can be recovered by
$\vectv^*=[\vectvt^*/\tilde{v}^*_{R+1}]_{(1:R)}$, where $[\vect{x}]_{(1:R)}$ denotes the first $R$ elements of vector $\vect{x}$ and $x_r$ denotes the $r$-th element of vector $\vect{x}$ \cite{IRSImprovement1}.

To deal with the non-convex constraints, the matrix lifting technique can be applied to obtain a convex formulation \cite{federatedLearning}. Specifically, by defining $\matV = \vectvt\vectvt^H$, the phase shift vector $\vectvt$ is lifted into a \ac{PSD} matrix $\mat{V}$.

By expressing $\Tr{\matM_{k,i}^o \matV}\, \hat{=}\, \vectvt^H\matM_{k,i}^o\vectvt$ and introducing the slack variables $\zeta_k^p$ and $\zeta_k^c$ problem (\ref{eq:genV-reform1}) can be expressed as $\underset{\phantom{|}}{ }$
\begin{align}\label{eq:genV-alpha}
&\underset{\matV,\{\zeta_k^p,\zeta_{k}^c\}_{k=1}^K}{\text{maximize}}\qquad \sum_{k \in \mathcal{K}} \eta_k^p\zeta_k^p + \eta_k^c\zeta_{k}^c  \tag{P3.2}\\
   &\text{subject to} \qquad
    \sqr{|b_{k,k}^p|} +  \Tr{\matM_{k,k}^p\matV} \geq  t_k^p \nonumber \\& \Big(
        \sum_{j\in\mathcal{K}\text{\textbackslash}\cbrackets{k}} \sqr{|b_{k,j}^p|} +  \Tr{\matM_{k,j}^p\matV}
          \sum_{\ell \in \Psi_k} \sqr{|b_{k,\ell}^c|} +  \nonumber \\ & \Tr{\matM_{k,\ell}^c \matV}  + \sigma^2 \Big) + \zeta_k^p,  \hspace{0.5cm} \forall k \in \mathcal{K}  \label{eq:SINR_p-reform5}\\
    &\sqr{|b_{i,k}^c|}+  \Tr{\matM_{i,k}^c \matV} \geq t_k^c \Big(
         \sum_{j \in \mathcal{K}}^{\phantom{I}} \sqr{|b_{i,j}^p|} +  \Tr{\matM_{i,j}^p\matV} \nonumber \\ & + \sigma^2   + \sum_{\ell \in \Psi_i} \sqr{|b_{i,\ell}^c|} + \Tr{\matM_{i,\ell}^c \matV} + \sum_{m \in \Omega_{i,k}} \sqr{|b_{i,m}^c|} + \nonumber \\ &  \Tr{\matM_{i,m}^c \matV} \Big) + \zeta_{k}^c,  \hspace{0.35cm} \forall k \in \mathcal{K} ,\, \forall i \in \mathcal{M}_k  \label{eq:SINR_c-reform5}\\
    & V_{r,r} = 1, \hspace{3.25cm}\forall r \in \{ 1,..., R+1\}\\
    & \matV \succeq 0  \label{eq:genV-alpha_last}\\
    &  \rank{\matV} =1 \label{eq:genV-reform5_nonConvex},
\end{align}
where $\zeta^p_k$ and $\zeta_{k}^p$ can be interpreted as \textit{SINR residuals} of user $k$ in phase shift optimization \cite{IRSImprovement1} and \begin{align}
\eta_k^o = {\underset{i\in \mathcal{N}}{\sum}{\myNorm{\vectw_{i,k}^o}_2^2}}\big/{\underset{k\in\mathcal{K}}{\max}\cbrackets{\displaystyle\sum_{i \in \mathcal{N}}\myNorm{\vectw_{i,k}^p}_2^2 ,\displaystyle\sum_{i \in \mathcal{N}}\myNorm{\vectw_{i,k}^c}_2^2}}
\end{align}
are weighting factors that prioritize users, which require high transmission power.
To reformulate the rank-one constraint, the following proposition is introduced:
\begin{prop}\label{prop:1}
 \textit{For a \ac{PSD} matrix $\mat{X} \in \mathbb{C}^{N\times N}$ and }$\myNorm{\mat{X}}_* \geq 0$\textit{, it holds \cite{federatedLearning} that}
\end{prop}
\begin{align}\label{eq:eqR1}
   \text{rank}(\mat{X}) = 1 \Leftrightarrow \myNorm{\mat{X}}_* - \myNorm{\mat{X}}_2 = 0,
\end{align}
\textit{where $\myNorm{\mat{X}}_*$ denotes the nuclear norm and $\myNorm{\mat{X}}_2$ denotes the spectral norm of $\mat{X}$.}\\
\\
Similar to the lower bounds derived in (\ref{DC-approxp}) and (\ref{DC-approxc}), the first-order Taylor approximation of the spectral norm $\myNorm{\mat{V}}_2$ around point $\mat{V}^0$ can be derived as
\begin{align}\label{convCons1}
   \myNorm{\mat{V}}_2 \geq \myNorm{\mat{V}^0}_2 + \langle \partial_{\mat{V}^0} \myNorm{\mat{V}}_2 , \sbrackets{\mat{V}-\mat{V}^0}\rangle,
\end{align}
where $\partial_{\mat{V}^0}$ is the subgradient of $\myNorm{\mat{V}}_2$ with respect to $\matV$ at $\matV^0$ and where the inner product is defined as
$\langle \mat{X},\mat{Y} \rangle = \text{Re}\cbrackets{\Tr{\mat{X}^H\mat{Y}}}$,
as stated by Wirtinger's calculus \cite{wirtingers} in the complex domain. Therefore, a convex approximation of (\ref{eq:eqR1}) can be established, by replacing the spectral norm with the approximation given in (\ref{convCons1}). By adding the resulting expression as a penalty term to problem (\ref{eq:genV-alpha}) the following optimization problem can be obtained
\begin{align}\label{eq:genV-alpha_rank}
   &\underset{\matV,\{\zeta_k^p,\zeta_{k}^c\}_{k=1}^K}{\text{maximize}} \quad \rho \Big( \sum_{k \in \mathcal{K}}  \hspace{-0.05cm} \eta_k^p\zeta_k^p + \eta_k^c\zeta_{k}^c \Big) - \,  (1-\rho)  \tag{P3.3}\\ & \hspace{1cm} \Big(\hspace{-0.05cm}\myNorm{\mat{V}}_* - \myNorm{\mat{V}^0}_2 - \langle \partial_{\mat{V}^0} \myNorm{\mat{V}}_2 , \sbrackets{\mat{V}-\mat{V}^0}\rangle\hspace{-0.05cm} \Big) \nonumber \\
   &\text{subject to} \hspace{0.5cm}  (\ref{eq:SINR_p-reform5}) - (\ref{eq:genV-alpha_last}),
\end{align}
where $\rho$ is a trade-off factor, that regulates, the trade-off between a high quality solution and a rank-one solution. It is worth noting, that the subgradient $\partial_{\mat{V}^0}\myNorm{\mat{V}}_2$ can be efficiently computed by using the following proposition \cite{federatedLearning}.
\begin{prop}\label{prop:2}
\textit{For a given \ac{PSD} matrix $\mat{X}\in\mathbb{C}^{N\times N} $, the subgradient  $\partial_{\mat{X}}\myNorm{\mat{X}}_2$ can be computed as $\vect{e}_1\vect{e}_1^H$, where $\vect{e}_1 \in \mathbb{C}^N$ is the leading eigenvector of matrix $\mat{X}$.}
\end{prop}

Since the retrieved solution may not be rank-one, the Gaussian randomization technique is used to obtain a feasible solution to problem (\ref{eq:genV-alpha_rank}). To this end, the \ac{SVD} is applied to the solution $\matV^*$ of problem (\ref{eq:genV-alpha_rank}) as
$\matV^* = \mat{U} \mat{\Sigma} \mat{U}^H$,
where $\mat{U} \in \mathbb{C}^{(R+1)\times(R+1)}$ and $\mat{\Sigma} \in \mathbb{C}^{(R+1)\times(R+1)}$ are a unitary matrix and a diagonal matrix, respectively. Using these \ac{SVD} components, a rank-one candidate solution $\hat{\vectv}_g$ to problem (\ref{eq:genV-reform1}) can be generated \cite{GaussRandHelp} as
\begin{align}\label{eq:candidate}
   \hat{\vectv}_g = \mat{U}\mat{\Sigma}^{\frac{1}{2}} \vect{z}_g \in \mathbb{C}^{(R+1)\times 1},
\end{align}
where $\vect{z}_g \sim \mathcal{CN}(\zero_{R+1},\mat{I}_{R+1})$ denotes a random vector drawn independently from a circularly-symmetric complex Gaussian distribution. After generating $G$ randomized solutions, each randomization $\hat{\vectv}_g$ can be used to obtain a potential candidate solution $\overline{\vectv}_g$ for problem (\ref{eq:genV-reform1}), namely
\begin{align}\label{eq:finalVsol}
   \displaystyle \overline{\vectv}_g = \exp\left({\displaystyle j \arg{ \sbrackets{ \hbrackets{{\hat{\vectv}}/{\hat{v}_{R+1}}}_{(1:R)}}  }}\right).
\end{align} Each potential candidate solution $\overline{\vectv}$, that satisfies problem (\ref{eq:genV-reform1}), is a feasible candidate solution. Since there is no objective function in problem (\ref{eq:genV-reform1}), the highest achievable sum-rate is chosen as a criterion in order to find the best performing beamforming vector. 



==> Publish5 v9 (conference-arxiv)/sections/alternatingMinimization/w_problem.tex <==
\section{Alternating Optimization}
To facilitate practical implementation, an alternating optimization framework is introduced to solve the problem in a distributed fashion. To this end, problem (\ref{eq:genProb}) is first reformulated into a form suitable for the inner-convex approximation framework \citep{AlaaRSCMD,Alaa_EE_RSCMD}, and second recasted into an semidefinite programming (SDP) problem.
\subsection{Beamforming Design}
In the initial step of the algorithm, $\vectv$ is assumed to be fixed, and consequently not an optimization variable. The optimization problem (\ref{eq:genProb}) can therefore be reformulated to
\begin{align}\label{eq:genW}
    &\underset{\{\vect{w}_k,\vect{t}_k,\mat{R}_k\}_{k=1}^K}{\text{minimize}} \qquad P(\vectw) \tag{P2.1}\\
    &\text{subject to} \quad  \nonumber \\
    &R_k^p + R_k^c \geq r_k^{Min} \label{eq:p2.1_first}\\
%    &\sum_{k \in \mathcal{K}_n^p}R_k^p + \sum_{k \in \mathcal{K}_n^c}R_k^c \leq C_n \,,\qquad \forall n \in \mathcal{N}\\
    & R_k^p - B \log_2(1+t_k^p) \leq 0\\
    & R_k^c - B \log_2(1+t_k^c) \leq 0\\
   &\vect{t}_k \geq 0\\
   &\mat{R}_k \geq 0 \label{eq:2.1_last}\\
   & t_k^p \leq  \gamma_k^p(\vectw),     \hspace{2.35cm} \forall k \in \mathcal{K} \label{eq:tkp}\\
   & t_k^c \leq  \gamma_{i,k}^c(\vectw), \hspace{2.175cm} \forall k \in \mathcal{K} ,\, \forall i \in \mathcal{M}_k, \label{eq:tkc}
\end{align}
where the variables $\mat{R}_k= \hbrackets{R_k^p,R_k^c}^T$ and $\vect{t}_k=\hbrackets{t_k^p,t_k^c}^T$ are introduced. $\vect{t}_k  \geq  0$ and $\mat{R}_k  \geq  0$ indicate that vector $\vect{t}_k$ and matrix $\mat{R}_k$ are greater than or equal to 0 in a component-wise manner.
The constraints (\ref{eq:tkp}) and (\ref{eq:tkc}) still define a non-convex feasible set, which makes problem (\ref{eq:genW}) non-convex. To overcome this challenge, equal representations of the constraints (\ref{eq:tkp}) and (\ref{eq:tkc}) are adopted, namely
\begin{align}\label{eq:tkp2}
         & {\sum_{m\in\mathcal{K}\text{\textbackslash}\cbrackets{k}}^{K} |\sbrackets{\vecth_k^{\text{eff}}}^H \vect{\omega}_m^p|^2 + \sum_{\ell \in \Psi_k} |\sbrackets{\vecth_k^{\text{eff}}}^H \vect{\omega}_\ell^c|^2 + \sigma^2}\, \nonumber \\ & \hspace{3.8cm}-\, {\frac{|\sbrackets{\vecth_k^{\text{eff}}}^H \vect{\omega}_k^p|^2}{t_k^p}}\leq 0
         \end{align}
         \begin{align}
         &{T_i + \sum_{\ell \in \Psi_i} |\sbrackets{\vecth_i^{\text{eff}}}^H \vect{\omega}_\ell^c|^2 \phantom{\frac{|}{|}} \hspace{-0.075cm} + \sum_{m \in \Omega_{i,k}} |\sbrackets{\vecth_i^{\text{eff}}}^H \vect{\omega}_m^c|^2}\,\ \nonumber \\ & \hspace{3.8cm} -\, {\frac{|\sbrackets{\vecth_i^{\text{eff}}}^H \vect{\omega}_k^c|^2}
         {t_k^c}} \leq 0 \label{eq:tkc2}    ,
   \end{align}
where with an abuse of notation the dependency of $\vect{h}_k^{\text{eff}}$ from $\vectv$ is skipped. The constraints are now represented in the form of difference-of-convex functions, which makes it possible to approximate them by using the first-order Taylor approximation around a feasible point $(\tilde{\vectw},\tilde{\vect{t}})$ \cite{convexFunct2,boyd_convex}.

To derive a lower bound for the second (negative) convex terms, the first-order Taylor approximation is applied.$\underset{\phantom{|}}{ }$ Therefore,
if $(\tilde{\vectw},\overset{\phantom{,}}{\tilde{\vect{t}})}$ is a feasible point of problem (\ref{eq:genW}) then it holds \cite{AlaaRSCMD}, that
\begin{align}\label{DC-approxp}
\frac{|\sbrackets{\vecth_k^{\text{eff}}}^H \vect{\omega}_k^p|^2}
{t_k^p} \geq&
\frac{2\Re\cbrackets{ \sbrackets{\tilde{\vect{\omega}}_k^p}^H \vecth_k^{\text{eff}} \sbrackets{\vecth_k^{\text{eff}}}^H \vect{\omega}_k^p}}
{\overset{}{\tilde{t}_k^p}} \nonumber \\
\hspace{3cm}&-
\frac{|\sbrackets{\vecth_k^{\text{eff}}}^H \overset{\phantom{I}}{\tilde{\vect{\omega}}_k^p}|^2}
{\sbrackets{\tilde{t}_k^p}^2} \, t_k^p
\end{align}
and
\begin{align}\label{DC-approxc}
\hspace{0.05cm}\frac{|\sbrackets{\vecth_i^{\text{eff}}}^H \vect{\omega}_k^c|^2}
{t_k^c} \geq&
\frac{2\Re\cbrackets{ \sbrackets{\tilde{\vect{\omega}}_k^c}^H \vecth_i^{\text{eff}} \sbrackets{\vecth_i^{\text{eff}}}^H \vect{\omega}_k^c}}
{\overset{}{\tilde{t}_k^c}} \nonumber \\
\hspace{3cm}&-
\frac{|\sbrackets{\vecth_i^{\text{eff}}}^H \overset{\phantom{I}}{\tilde{\vect{\omega}}_k^c}|^2}
{\sbrackets{\tilde{t}_k^c}^2} \, t_k^c ,
\end{align}
where $\text{Re}\cbrackets{\cdot}$ denotes the real part of a complex-valued number.
The approximations (\ref{DC-approxp}) and (\ref{DC-approxc}) can be utilized to establish inner-convex subsets by substituting the corresponding terms in (\ref{eq:tkp2}) and (\ref{eq:tkc2}) with their respective lower bound, namely
\begin{align}
      &0 \geq \sum_{j\in\mathcal{K}\text{\textbackslash}\cbrackets{k}} |\sbrackets{\vecth_k^{\text{eff}}}^H \vect{\omega}_j^p|^2 + \sum_{\ell \in \Psi_k} |\sbrackets{\vecth_k^{\text{eff}}}^H \vect{\omega}_\ell^c|^2 + \sigma^2-
      \nonumber\\
      &\frac{2\Re\cbrackets{ \sbrackets{\tilde{\vect{\omega}}_k^p}^H \vecth_k^{\text{eff}} \sbrackets{\vecth_k^{\text{eff}}}^H \vect{\omega}_k^p}}
      {\overset{}{\tilde{t}_k^p}}+\frac{|\sbrackets{\vecth_k^{\text{eff}}}^H \overset{\phantom{I}}{\tilde{\vect{\omega}}_k^p}|^2}
      {\sbrackets{\tilde{t}_k^p}^2} \, t_k^p,\forall k \in \mathcal{K}  \nonumber \\
       \label{eq:approxCon1}\\
      &0\geq {T_i}+ \sum_{\ell \in \Psi_i} |\sbrackets{\vecth_i^{\text{eff}}}^H \vect{\omega}_\ell^c|^2 + \sum_{m \in \Omega_{i,k}} |\sbrackets{\vecth_i^{\text{eff}}}^H \vect{\omega}_m^c|^2-
      \nonumber \\
      &\frac{2\Re\cbrackets{ \sbrackets{\tilde{\vect{\omega}}_k^c}^H \vecth_i^{\text{eff}} \sbrackets{\vecth_i^{\text{eff}}}^H \vect{\omega}_k^c}}
      {\overset{}{\tilde{t}_k^c}}+ \frac{|\sbrackets{\vecth_i^{\text{eff}}}^H \overset{\phantom{I}}{\tilde{\vect{\omega}}_k^c}|^2}
      {\sbrackets{\tilde{t}_k^c}^2} \, t_k^c, \nonumber \\ &\hspace{6cm}\forall k \in \mathcal{K} ,\, \forall i \in \mathcal{M}_k .   \nonumber \\
     \label{eq:approxCon2}
\end{align}
Thus, we have the following convex optimization problem
 \begin{align}\label{eq:cmpW}
   & \underset{ \{\vect{w}_k,\vect{t}_k,\mat{R}_k\}_{k=1}^K}{\text{min}}\quad  \sum_{k\in \mathcal{K}} P(\vect{\omega}) \tag{P2.2}\\
   & \text{subject to} \qquad \nonumber\\
   &(\ref{eq:p2.1_first})-(\ref{eq:tkc}),\,(\ref{eq:approxCon1}),\,(\ref{eq:approxCon2}).\nonumber
\end{align}
Problem (\ref{eq:cmpW}) is convex and can be solved with standard optimization tools. Moreover, let $\mat{\Lambda} = \hbrackets{\vect{w}^T ,\,\vect{t}^T}^T$ be a vector stacking the optimization variables of (\ref{eq:cmpW}), $\widehat{\mat{\Lambda}}_z = \hbrackets{ \widehat{\vect{w}}_z^T ,\, \widehat{\vect{t}}_z^{\,\,T}\,}^T $ be the variables that are the optimal solution of problem (\ref{eq:cmpW}) computed at iteration $z$ and $\tilde{\mat{\Lambda}} = \hbrackets{ \tilde{\vect{w}}^T ,\, \tilde{\vect{t}}\phantom{.}^T\,}^T $ be the point, around which the approximations are computed. First, vector $\tilde{\mat{\Lambda}}$ is initialized by finding feasible \ac{MRC} beamformers $\tilde{\vect{w}}$ for the users. Using the initialization, can be solved to obtain the vector $\widehat{\mat{\Lambda}}_z$. If the current solution is not stationary,$\underset{\phantom{|}}{ }$ it is used for computing $\overset{\phantom{.}}{\tilde{\mat{\Lambda}}}$ for the next iteration, i.e. $\tilde{\mat{\Lambda}}_{z+1} = \tilde{\mat{\Lambda}}_z + \varrho_z \sbrackets{\widehat{\mat{\Lambda}}_z - \tilde{\mat{\Lambda}}_z},\,\text{for some }\varrho_z \in (0,1]$






==> Publish5 v9 (conference-arxiv)/sections/conclusion.tex <==
\section{Conclusion}\label{ch:conc}
B5G networks are forecast to be dense networks that suffer from high interference but simultaneously require high data rates. With the goal to minimize the total transmit power consumption of the network, subject to per-user \ac{QoS} constraints, the \ac{IRS}-assisted \ac{C-RAN} is combined with the \ac{RS} scheme in order to mitigate the interference within the network. This also includes the interference amplified by the \ac{IRS}, which is caused by the optimization of the phase shifts towards the weaker users. To study the effect of this synergistic interaction between the \ac{RS} scheme and the \ac{IRS} on the reduction of the total required transmit power, an optimization problem is formulated. An alternating optimization approach is proposed to decouple the problem into two subproblems. As the resulting subproblems still remain non-convex, two frameworks are proposed, that obtain sub-optimal solutions to these subproblems. Results show that the combination of the \ac{IRS} with the \ac{RS} scheme can significantly decrease the required network power consumption as the \ac{RS} scheme is able to mitigate interference within the network, including the \ac{IRS}-assisted interference. In fact, the power savings, obtained by combining both techniques, exceed the sum of the power savings, that each technique can achieve individually. 

==> Publish5 v9 (conference-arxiv)/sections/convergence_behaviour.tex <==
\section{Numerical Simulations}\label{ch:numsim}
The simulation setup considers a \ac{C-RAN}, which consists of one \ac{CP}, that is connected to 4 \acp{BS} via fronthaul links. Each \ac{BS} is equipped with 4 antennas. The \acp{BS} operate in an area of $[-500,500] \times [-500,500] \text{ m}^2 $ and serve 6 single-antenna users. We also consider placing an \ac{IRS} in the center of this squared area, which consists of $R=15$$\underset{\phantom{|}}{ }$reflecting elements. The users and \acp{BS} are positioned uniformly and independently within the operation area. The channels between the \acp{BS}, users and \ac{IRS} follows the standard path-loss model consisting of three components: 1) path-loss as $\text{PL}_{x,y} = 148.1 + 37.6\log_{10}(d_{x,y})$, where $d_{x,y}$ is the distance between transmitter $x$ and receiver $y$ in km; 2) log-normal shadowing with 8dB standard deviation and 3) Rayleigh channel fading with zero-mean and unit-variance. The transmit bandwidth is assumed to be $B=10$ MHz, the noise power spectrum is set to -169 dBm/Hz and the minimum \ac{QoS} is set to $r_k^{\text{Min}}=4$ Mbps for each user. The sum-power weights $\alpha_k$ of the users are chosen in a uniform fashion, i.e. $\alpha_k \sim \mathcal{U}(1,2)$. It is assumed that the clusters are determined as $\mathcal{K}_n^p=\mathcal{K}_n^c=\mathcal{K},\, \forall n \in \mathcal{N}$. Furthermore, the number of Gaussian randomizations is set to $G=25$, the trade-off parameter is set to $\rho=0.9$ and $D=2$. 

==> Publish5 v9 (conference-arxiv)/sections/introduction.tex <==
\section{Introduction}
With the introduction of solutions based on the \ac{IoT} on various application areas, such as healthcare, industrial control etc., billions of new devices with different applications will connect to \ac{B5G} wireless networks \cite{microsoftIoT}, which naturally results in an increase in interference. Furthermore, more \acp{BS} are deployed within each cell, due to the utilization of the spatial reuse technique, which also increases inter-cell interference. To tackle the challenges of modern communication networks, \acp{IRS} have been shown to be a promising cost-effective solution to increase the achievable data rates of existing wireless networks by improving the spectral efficiency and the signal coverage \citep{,IRS_intr2,IRS_intr4}. The \ac{IRS} is a physical reflective metasurface consisting of small reflect elements, whose changes to the reflected signal can be controlled independently by a smart controller. The deployment of an \ac{IRS} therefore enables the possibility to smartly reflect incident waves and simultaneously adjust the phase shift of each reflect element. Consequently, the \ac{IRS} is able to add phase shifts at the user either constructively, thus improving the received signal power, or destructively, and thus mitigating interference. However, the changes to the reflected signals do not result in an improvement for all \ac{IRS}-assisted transmissions. Therefore, the \ac{IRS} is not only amplifying the received signal, but also the received interference for most users, especially in dense networks. 

For this reason, this paper utilizes the \ac{RS} technique, which is able to  mitigate interference within the network in such a way that the interference, amplified by the \ac{IRS}, is also mitigated. To enable the practical implementation of the \ac{RS} scheme, a \ac{C-RAN} setting is adopted \citep{Alaa_EE_RSCMD,Alaa_27}, in which the central processor at the cloud is connected to a set of \acp{BS} via high-speed and high-capacity fronthaul links \cite{C-RAN}, while simultaneously adjusting the \ac{IRS}. 

To study the effect of both techniques on the minimum required transmit power, we investigate the optimal power control in the \ac{IRS}-assisted and RS-enabled \ac{C-RAN} to minimize the required transmit power under per-user minimum \ac{QoS} constraints. This poses a challenging optimization problem due to the coupling of the optimization variables in the non-convex \ac{QoS} constraints. Therefore, an alternating optimization framework is proposed, which decouples the variables and solves the emerging sub-problems alternatively. The results obtained are compared with a baseline scheme of \ac{TIN} \citep{5074583,jabar}.

==> Publish5 v9 (conference-arxiv)/sections/numerical_results.tex <==

Figure \ref{fig:normQoS} illustrates the normalized transmit power for different \ac{QoS} requirements of each user normalized to $r_k^{\text{Min}}$. The figure shows that the slopes of the lines, which represent the \ac{RS} schemes are smaller than the slopes of the lines of the respective \ac{TIN} scheme, which highlights the efficiency of the \ac{RS} scheme compared to \ac{TIN}. Deploying an \ac{IRS} lowers the required transmit power by around 5 dBm/Mbps if compared to the non-\ac{IRS} cases. Interestingly the performance gain of \ac{RS} compared with \ac{TIN} becomes larger when using an \ac{IRS}. Intuitively, with an \ac{IRS} the channel quality of all users significantly improves, however, this also leads to substantial interference increase. Hence, the RS gain becomes more pronounced in such a case.
\begin{figure}
\hspace{-0.65cm}\includegraphics[width = 1.15\columnwidth]{figure2}
\caption{The normalized minimum required transmit power to satisfy the \ac{QoS} requirements of the users.}
\label{fig:normQoS}
\end{figure} 



==> Publish5 v9 (conference-arxiv)/sections/preliminaries.tex <==
\section{Power Minimization Techniques}\label{ch:PowMin}
\input{sections/preliminaries/rate_splitting.tex}
\input{sections/preliminaries/intelligent_reflective_surface}


==> Publish5 v9 (conference-arxiv)/sections/preliminaries/intelligent_reflective_surface.tex <==
\subsection{Intelligent Reflecting Surface}
Since the beginning of wireless communication networks, the medium between the transmitter and receiver has been modeled as a randomly behaving entity. The randomness of the surroundings, which the transmitted radio waves are subjected to and uncontrollably interacting with, causes the quality of received signal to degrade.\\
Intelligent reflecting surfaces, also known as Large Intelligent Surfaces, Intelligent Reconfigurable Surfaces, Software-controlled Metasurfaces and more, comprise an array of reflect elements, that are able to influence, and consequently control the \nohyphens{reflection} of the incident signal. The change of the reflected signal may be about the amplitude, phase, frequency and polarization \cite{IRSTheoPerfLim}. As each reflect element can be independently controlled by a smart controller, the IRS is able control the wireless propagation environment to establish favourable channel responses. Therefore, the IRS is able to generate controllable passive beamforming as depicted in Figure \ref{fig:IRSsimple}.\\
\\
The \ac{IRS} and its controllable reflect elements can be modeled as depicted in Figure \ref{fig:IRSModel}, where an IRS consisting of $R$ reflect elements is considered. The figure shows that each antenna of the transmitter has a channel $h_r$ to each reflect element of the IRS and a direct channel $h_0$ to the user. At the IRS, the induced changes on the incident signal caused by $r$-th reflect element are captured with the reflection coefficient $v_r$. After inducing the changes, each reflect element reflects the signal to the receiver through a channel $g_r$. It is noted that the channels $g_r$ from the IRS to the receiver differ from the channels $h_r$ between the IRS and the transmitter. The change of amplitude $\beta_r$ and phase $e^{j\theta_r}$ on the reflected signal caused by the $r$-th reflect element could therefore be represented by defining its reflection coefficient as $v_r = \beta_r e^{j\theta_r}$ .\\
\begin{figure}
\centering
\includegraphics[width=\columnwidth]{pictures/IRS_simple}
\caption{Intelligent Reflecting Surface (\ac{IRS})}
\label{fig:IRSsimple}
\end{figure}
\begin{figure}
\centering
\includegraphics[width=\columnwidth]{pictures/IRS-modell}
\caption{Model of an intelligent reflecting surface with $R$ reflect elements, where $h_0$ represents the channel of the direct \ac{LoS} path between transmitter and receiver and $v_r$ represents the reflect coefficient of the $r$-th element.}
\label{fig:IRSModel}
\end{figure}
The first concept of a reflecting surface in wireless communication systems dates back to 1963, in which the reflecting elements of a \textit{Reflectarray}  were mounted directly to the antenna in order to generate different radiation patterns \cite{ReflectArray}. Recent advancements, however, made it possible to reconfigure the changes on the incident signal in real time \cite{IRSrealtimeChange1,IRSrealtimeChange2},
which made the use of \ac{IRS}s applicable in modern wireless communication systems \cite{AnasIRSImprovement,IRSImprovement1,IRS_EEvsRelay,AnasIRSAnalysis}. In recent works, the changes induced to the incident signal by the \ac{IRS} are assumed to be phase shifts \cite{IRS_EEvsRelay,IRS_MIMO+Transmission}, which implies that the \ac{IRS} is passive in its ideal form, and therefore does not consume any of the available transmit power. However, since the phase shifts, that the \ac{IRS} induces, need to be adjusted regularly in order to positively impact the changing transmission scenarios, the \ac{IRS} requires a control signal, and consequently active components like the smart controller for adaptive phase shifting.\\
By correctly aligning its phase shifts, the \ac{IRS} is able to superposition phase shifts at the receiver to achieve either constructive interference to improve data rates or destructive interference to remove interference \cite{AnasIRSImprovement,IRSImprovement1,IRS_EEvsRelay}. The latter is also useful for enhancing security and privacy, which can be achieved by improving the physical layer security as the reflected signals can be configured to cancel out the \ac{BS}-to-eavesdropper \ac{LoS} signals. This effectively reduces the information leakage \cite{IRSpositioning}.\\ \\
Contrary to the first concept, \ac{IRS}s can be easily deployed on walls, buildings and ceilings of any shape, indoors and outdoors \cite{IRS_MIMO+Pos} because they can be practically fabricated to any arbitrary shaped surface, due to the modularity of the reflect elements \cite{IRSpositioning}. Moreover, the extension of any wireless network with \ac{IRS}s can be done without any major modification in the hardware and software of user equipment because the users effectively benefit from amplified channels.\\
\\
For obtaining an optimal transmission environment, the transmitter needs to be able to send a control signal to the \ac{IRS}. In recent works \cite{AnasIRSAnalysis,IRSImprovement1,IRScontroller,IRScontrollerII}, which study single-cell \ac{IRS}-assisted scenarios, a fronthaul link is employed, that connects the transmitter to a smart controller, which tunes the \ac{IRS} reflect elements based on the received signal. Because of the \ac{IRS}-assisted \ac{C-RAN} employed in this work, the central processor of the cloud is able to assume the tasks of the smart controller.\\
\\
%Figure \ref{fig:IRS-CRAN} depicts a simple \ac{IRS}-assisted \ac{C-RAN} transmission scenario with two users and two base stations, where the central processor of the cloud manages the control signal for the \ac{IRS} adjustments. The cloud also distributes the requested messages to the base stations, which then transmit the signals in the \ac{IRS}-enhanced environment. It is noted, that the \ac{IRS} reflects the transmit signals of each base station in reach to each user in reach. Hence, the reflected signal, that each user receives, can carry a desired and undesired part for the respective user and thus can either improve or deteriorate the users signal to interference and noise ratios, based on the current \ac{IRS} setting. Therefore, finding the optimal setting for the reflect elements of the \ac{IRS} is a crucial task for the improvement of  \ac{IRS}-assisted transmission scenarios. \\
Due to the similarities to relays in forwarding received signals, the performance of \ac{IRS}s can be compared to the performance of relays \cite{AnasIRSAnalysis,RelayIntelligentRS,bjornsonIRS}. In \cite{bjornsonIRS} it was shown that while decode-and-forward (DF) relaying suffers from pre-log penalty due to the two-hop transmission, the reflections from the \ac{IRS} must travel over two channels, from the transmitter to the \ac{IRS} and from the \ac{IRS} to the receiver, to reach the destination. This leads to a very small channel gain per reflect element of the \ac{IRS}. To meet the performance of the relay, many reflect elements have to be employed in order to counteract the low channel gain. However, even with hundreds of elements, the \ac{IRS} can still be of relatively small size because each reflect element is assumed to have a sub-wavelength size \cite{smallSize1,smallSize2} and can still remain cost-effective because the production cost of the reflect elements is low. Contrary to relays, there are no power amplifiers needed for the \ac{IRS} in its ideal form, which also means that there is no new interference introduced when using \acp{IRS} to improve the transmission scenario. Moreover, it has been shown that \acp{IRS} are able to significantly decrease network power consumption \cite{IRS_powerconsumpt} if deployed to aid wireless communication systems. Therefore, an \ac{IRS} can be more energy efficient than regular multi-antenna amplify-and-forward relaying \cite{IRS_EEvsRelay,bjornsonIRS}. However, even if deploying an \ac{IRS} is not the most efficient or effective solution, the low cost and versatility regarding deployment locations still makes the \ac{IRS} a viable alternative.\\
Another challenge that arises with the use of \acp{IRS} in communication systems is the need for new communication-theoretic models \cite{newComTheoModels}. In fact, in current wireless networks the devices and transmission protocols are designed to adapt themselves to the current transmission scenario. In this case, the devices are the endpoints of the communication environment, which is treated as unintentional and uncertain interference to the transmission. Incorporating an \ac{IRS} to the communication scenario adds another degree of freedom to the transmission scenario and enables the environment to behave smartly \cite{newComTheoModels}.
%Hence, instead of optimizing only the endpoints, i.e transmitter and receiver, Smart Radio Environments can be configured dynamically and support the transmission scenario \cite{newComTheoModels}.


==> Publish5 v9 (conference-arxiv)/sections/preliminaries/rate_splitting.tex <==
\subsection{Rate Splitting and Common Message Decoding}
Delivering different types of messages to different types of users has been of great interest with the emerging technologies and appliances of \ac{IoT}. Furthermore, with the deployment of more devices into small cells, the distances between the users and \acp{BS} decreases. As a consequence, the direct \ac{LoS} channels become stronger and of better quality to the detriment of increasing inter-BS interference because of close proximity of \acp{BS} in neighbouring cells. For conventional transmission schemes, which use treating interference as noise as strategy, these changes to the transmission scenario degrade the overall network performance significantly, especially in already interference-limited dense networks \cite{aydin-sub-opt,aydin-crystal}.\\
\\
In contrast to \ac{TIN}, the \ac{RS-CMD} strategy for the two-user \ac{IC} consists of splitting the messages of each user into two parts, a private part, that is decoded by the intended user only, and a common part, that can be decoded at both, the intended user as well as the interfered user in the network  \cite{RS-Base}. This scenario is depicted in Figure \ref{fig:RSsimple}, where each \ac{BS} splits the message of its allocated user into a common and private part. The figure shows that user $1$ receives the private and common messages of both users. However, user $1$ is able to decode the common message $\hat{s}_2^c$ of user $2$ before decoding its own common and private message $\hat{s}_1^c$ and $\hat{s}_1^p$. The ability to decode the common message of other users enables both users to cancel out a part of their received interference. Figure \ref{fig:RSsimple2} shows the \ac{SIC} receiver at user $1$, which enables mitigating the interference caused by the common message $\hat{s}_2^c$ of user $2$ by applying \ac{SIC}. Therefore, using the \ac{RS-CMD} strategy can increase the achievable data rates when compared to the TIN strategy. In fact, for the two-user \ac{IC} it has been shown, that the \ac{TIN} strategy is suboptimal \citep{RS-Base,Kobayashi,WithinOneBit,CapacityAydin}, while the \ac{RS-CMD} strategy has been shown to approach the largest capacity region of the \ac{IC} to within one bit \cite{Kobayashi,WithinOneBit}.
\begin{figure}
\centering
   \includegraphics[scale=0.9]{pictures/rate-splitting_simple_nc}
   \caption{\ac{RS-CMD} strategy for the two-user IC. Each \ac{BS} splits the message of its allocated user into a private and common part.}
\label{fig:RSsimple}
\end{figure}
\begin{figure}
\centering
   \includegraphics[scale=1.1]{pictures/rate-splitting_simple_nc2}
   \caption{Successive Interference Cancellation Receiver at User 1}
\label{fig:RSsimple2}
\end{figure}
The idea of splitting the messages of each user with the intent to mitigate interference can be extended to a scenario with multiple users, in which the common parts are decoded by a selected group of receivers with the aim of mitigating interference within this group. To ensure that each user in this group is able to decode the same common message, the achievable common rate of each user in this group, decoding the common message of this group, has to be equal. For this reason, finding suitable groups of users, which decode the same common messages, is an important task for determining the gain of \ac{RS-CMD} over \ac{TIN} \cite{AlaaRSCMD}. Furthermore, more layers of the successive decoding strategy at the receivers can be employed \cite{AlaaRS,AlaaRSCMD}, which improves the performance of \ac{RS-CMD} for dense networks, in which each receiver is subjected to multiple sources of interference. Hence, \ac{RS-CMD} provides a high flexibility with regards to the allocation of rates, beamforming design and range of decoding layers and can provide a significant improvement in performance, especially in dense networks. In fact, it has been shown that rate splitting is a generalization of classical linear precoding methods and is able to improve the spectral efficiency in downlink broadcast channels considerably \cite{gen_linprecoder}. Moreover, applying  \ac{RS-CMD} beyond the two-user interference channel to a multi-cell multiuser downlink scenario, subject to minimum achievable rate constraints across the users, has been shown to bring substantial benefit in terms of improving the maximum minimal rate, especially for cell-edge users as they are able to mitigate inter-cell interference \cite{RS-Theo2Prax}.\\
\\
However, in rate splitting, the cooperation of multiple \acp{BS} is required in order to deliver the private and common messages to the users because the messages have to be split and encoded jointly. In fact, the transmitted signals at the \acp{BS} are designed as superpositions of the private and common messages. Therefore, a suitable platform for the physical implementation of rate splitting techniques is the \ac{C-RAN} architecture, which is able to virtualize baseband functionalities to a centralized cloud entity. This central processor (\ac{CP}) is connected to the \acp{BS} in the cloud-enabled network and facilitates centralized processing, that can be utilized to apply enhanced interference management techniques, which are superior to classical interference management techniques in \ac{MIMO} networks \cite{MIMO-CRAN-interference-mitigation,AlaaRS,AlaaRSCMD}. Due to this hierarchy, the \ac{CP} is able to jointly encode the messages for each user and design the transmit signals for cooperating clusters of \acp{BS}, subject to per-user \ac{QoS} constraints, with the aim to maximize the interference mitigation effects. It has been shown that using \ac{RS-CMD} in combination with the \ac{C-RAN} architecture, in order to mitigate interference, provides a significant gain if compared to interference mitigation techniques, that do not rely on \ac{RS-CMD} \cite{AlaaRSCMD}. In fact, it has been shown that the use of \ac{RS-CMD} in \ac{MIMO} \ac{C-RAN} systems can achieve gains of up to 97\% in terms of the energy efficiency \cite{Alaa_EE_RSCMD} and 27\% in terms of the achievable maximum sum-rate \cite{Alaa_27} over the baseline scheme of treating interference as noise.




==> Publish5 v9 (conference-arxiv)/sections/problem_formulation.tex <==
\section{Problem Formulation}\label{ch:propform}
\input{sections/problem_formulation/general_problem.tex}


==> Publish5 v9 (conference-arxiv)/sections/problem_formulation/general_problem.tex <==
Let the total transmit power be defined as
\begin{align}\label{eq:Ptr}
  P(\vectw) & =  \sum_{k\in \mathcal{K}}  \alpha_k \left( \sum_{n\in \mathcal{N}} \myNorm{ \vect{\omega}_{n,k}^p}_2^2 \ + \myNorm{ \vect{\omega}_{n,k}^c}_2^2 \right),
\end{align}
where $\alpha_k$ is a weighting factor, which represents the priority of serving user $k$ compared to other users in the network.
\noindent
The problem can then be defined as
\begin{align}\label{eq:genProb}
   &\underset{\vectw,\vectv}{\text{minimize}} \quad P(\vectw) \tag{P1}\\
   &\text{subject to} \quad \nonumber \\ &\log_2\sbrackets{1+\gamma_k^p(\vectw,\vectv)}+ \nonumber\\
   &\underset{i \in \mathcal{M}_k}{\min} \cbrackets{ \log_2\sbrackets{1+\gamma_{i,k}^c\sbrackets{\vectw,\vectv}}} \geq r_k^{\text{Min}}/B ,\,   \forall k \in \mathcal{K}\label{eq:general_Minrate}\\
   &|v_r| = 1, \hspace{3.75cm}  \forall r \in \cbrackets{1,...,R},\label{eq:general_IRS}
\end{align}
where the constraints $0\leq \theta_r \leq 2\pi, \forall r\in\{1,...,R\}$ are represented by the equivalent unit modulus constraints in (\ref{eq:general_IRS}).
The problem is generally difficult to solve, due to the non-convex constraints (\ref{eq:general_Minrate}) and (\ref{eq:general_IRS}). Furthermore, the optimization variables are coupled in the \ac{QoS}$\underset{\phantom{|}}{ }$constraints (\ref{eq:general_Minrate}).









==> Publish5 v9 (conference-arxiv)/sections/system_model.tex <==
\section{System Model}\label{ch:Sysmod}

The system model considered in this work is depicted in Figure \ref{fig:IRS-CRAN} and consists of a \ac{RS}-enabled and \ac{IRS}-assisted \ac{C-RAN} downlink system. In more details, the network consists of a set of multi-antenna \acp{BS} $\mathcal{N} = \{1,2,\cdots,N\}$, each of which is equipped with $L \geq 1$ antennas. The \acp{BS} serve a set of single-antenna users $\mathcal{K} = \{1,2,\cdots,K\}$. An \ac{IRS}, composed of $R$ passive real-time-controllable reflect elements, is deployed in the communication environment to assist the \acp{BS} in their communication with the users. Each \ac{BS} $n \in \mathcal{N}$ is connected to the \ac{CP} at the cloud via orthogonal fronthaul links of unlimited capacity. Each user $k$ requires to be served with a minimum data rate $r_k^{\text{Min}}$, which represents the \ac{QoS} target of user $k$.

The channel vector, denoted by ${\vect{h}_{n,k} \in \mathbb{C}^{L\times1}}$, represents the direct channel links between \ac{BS} $n$ and user $k$. The channels of the \ac{IRS}-assisted path are composed of $\mat{H}_{n}^\text{BI} \in \mathbb{C}^{L \times R}$ and $\vecth_{k}^\text{IU} \in \mathbb{C}^{R \times 1}$ as depicted in Figure \ref{fig:IRS-CRAN}.
\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figure1}
\caption{IRS-assisted multiuser \ac{C-RAN} system}
\label{fig:IRS-CRAN}
\end{figure}
Let $\vect{h}_k = \left[ ({\vect{h}_{1,k}})^{\,T } ,({\vect{h}_{2,k}})^T, \dots ,({\vect{h}_{N,k}})^T \right]^T  \in \mathbb{C}^{NL\times1}$ be the aggregate direct channel vector of user $k$, $\vect{H}^{\text{BI}} = \left[ ({\vect{H}_{1}^{\text{BI}}})^{\,T } ,({\vect{H}_{2}^{\text{BI}}})^T, \dots ,({\vect{H}_{N}^{\text{BI}}})^T \right]^T  \in \mathbb{C}^{NL\times R}$ be the aggregate channel matrix from the \acp{BS} to the \ac{IRS} and $\vect{x} = \left[ {\vect{x}_{1}}^{\,T } ,{\vect{x}_{2}}^T, \dots , {\vect{x}_{N}}^T \right]^T  \in \mathbb{C}^{NL\times1}$ be the aggregate transmit signal vector. Using this notation, the received signal at user $k$ can be written as
\begin{align}\label{eq:recSig}
    y_k & = (\vect{h}_{k})^H\, \vect{x} + (\mat{H}^\text{BI} \, \mat{\Theta} \, \vect{h}_{k}^{\text{IU}})^H \, \vect{x} + n_k,
%       &= (\vect{h}_{k}^\text{BU} + \mat{H}^\text{BI} \, \mat{\Theta} \, \vect{h}_{k}^{\text{IU}})^H \, \vect{x} + n_k, \label{eq:recSig_pre}\\
\end{align}
where $n_k \sim \mathcal{CN}(0,\sigma^2)$ is the \ac{AWGN}, $\mat{\Theta}\, = \text{diag}(\vectv) \in \mathbb{C}^{R \times R}$ is a diagonal reflection coefficient matrix accounting for the response of the reflect elements. Let the phase shift vector be defined as $\vectv = [v_{1}, v_{2} , \dots v_{R}]^T$, where each reflection coefficient $v_r$ consists of a phase shift $\theta \in [0,2\pi]$, namely $v_r = e^{j\theta_r}$. By introducing the matrix $\matH_k = \matH^{\text{BI}}\, \text{diag}(\vecth_k^{\text{IU}})$ and denoting the sum of the aggregated direct and reflected channel vectors of user $k$ as an effective channel
$\vecth_k^{\text{eff}}(\vectv) = \vect{h}_{k} + \mat{H}_k \vectv$, the received signal (\ref{eq:recSig}) can be rewritten as $y_k  = (\vect{h}_k^{\text{eff}}(\vectv))^H \, \vect{x} + n_k$,



==> Publish5 v9 (conference-arxiv)/sections/transmission_scheme.tex <==
\subsection{Rate Splitting}
The \ac{CP} splits $q_k$, the requested message of user $k$, into two sub-messages, namely a private part $q_k^p$ and a common part $q_k^c$. Subsequently, the respective parts are encoded by the \ac{CP} into the private and common symbols $s_k^p$ and $s_k^c$, respectively. The coded symbols $s_k^p$ and $s_k^c$ are assumed to form an \ac{i.i.d.} Gaussian codebook. The \ac{CP} shares the private symbols $s_k^p$ (common symbols $s_k^c$) with a cluster of predetermined \acp{BS}, that exclusively send the beamformed private (common) symbols to user $k$. Given these definitions, the subset of users that are served by \ac{BS} $n$ with a private or common message $\mathcal{K}_n^p,\,\mathcal{K}_n^c \subseteq \mathcal{K}$, respectively, are defined by
\begin{align}
   \mathcal{K}_n^p &= \{k\in\mathcal{K} \, | \, \text{BS } n \text{ serves } s_k^p \text{ to user }k\},\\
   \mathcal{K}_n^c &= \{k\in\mathcal{K} \, | \, \text{BS } n \text{ serves } s_k^c \text{ to user }k\}.
\end{align}
The beamformers $\vectw_{n,k}^p$ and $\vectw_{n,k}^c$ used by \ac{BS} $n$ to send $s_k^p$ and $s_k^c$, respectively,  are created by the \ac{CP} and forwarded to \ac{BS} $n$ through the fronthaul link along with the respective private symbols $\cbrackets{s_k^p \,|\, \forall k \in \mathcal{K}_n^p}$ and common symbols $\cbrackets{s_k^c \,|\, \forall k \in \mathcal{K}_n^c}$.
After \ac{BS} $n$ receives the corresponding messages and beamformers, it constructs the transmit signal vector $\vect{x}_n$ and sends it to the users of interest. By denoting the aggregate beamforming vectors as $\vectw_k^o = \left[ (\vectw_{1,k}^o)^T,(\vectw_{2,k}^o)^T,\dots,(\vectw_{N,k}^o)^T  \right]^T  \in \mathbb{C}^{NL\times1}, \forall \, o \in \{p,c\}$ associated with $s_k^p$ and $s_k^c$, respectively, the aggregate transmit signal vector can be expressed as \begin{align}
\vect{x} = \sum_{k \in \mathcal{K}_n^p}\vectw_k^p s_k^p + \sum_{k \in \mathcal{K}_n^c}\vectw_k^c s_k^c.
\end{align}
Consequently, should \ac{BS} $n$ not participate in the cooperative transmission of the private or common symbol of user $k$, the respective beamformers are set to zero, namely $\vectw_{n,k}^p = \zero_L$ or $\vectw_{n,k}^c = \zero_L$, where $\zero_L$ denotes a column vector of length $L$ with all zero entries.

\subsection{Achievable rates}
In this work, the influence of the \ac{CMD} scheme, adopted by the users, is utilized for the purpose of interference mitigation. Hence, a successive decoding strategy is adopted, in which user $k$ decodes the common message of the user with the strongest channel (in the Euclidean norm sense) first. Let $\mathcal{M}_k$ be the set of users that decode $s_k^c$, i.e.,
\begin{align}
\mathcal{M}_k = \cbrackets{j \in \mathcal{K} \,|\, \text{ user } j \text{ decodes }s_k^c}.
\end{align}
In conjunction, let the set of users $\Phi_k$, whose common messages are decoded by user $k$, and the set of users $\Psi_k$, whose common messages are \textit{not} decoded by user $k$, be defined as
\begin{align}
\Phi_k = \cbrackets{j \in \mathcal{K} \, | \, k \in\mathcal{M}_j},\, \Psi_k = \cbrackets{j \notin \mathcal{K} \, | \, k \in\mathcal{M}_j},
\end{align}
respectively. It is noted that $\Phi_k$ and $\Psi_k$ are two disjoint subsets from the set of active users $\mathcal{K}$, while the cardinality of $\Phi_k$ is bounded by $D$, i.e., $|\Phi_k| \leq D.$ For the sets $\Phi_k ,\, \forall k\in\mathcal{K}$ a decoding order is established, which is represented by a mapping of an ordered set with cardinality of $|\Phi_k|$, i.e.,
\begin{align}
   \pi_k(j) : \cbrackets{1,2,\dots,|\Phi_k|} \rightarrow \Phi_k.
\end{align}
Assuming user $k$ decodes the common messages of user $j_1$ and user $j_2$ with $j_1 \neq j_2$, then $\pi_k(j_1) > \pi_k(j_2)$ implies that user $k$ decodes the common message of user $j_1$ first and the common message of user $j_2$ afterwards.
Furthermore, the set $\Omega_{i,k}$ is defined as
\begin{align}
   \Omega_{i,k} = \cbrackets{m\in\Phi_i \, | \, \pi_i(k) > \pi_i(m)}
\end{align}
and represents the set of users whose common messages are decoded by user $i$ after decoding the common message of user $k$.

Now, the received signal at user $k$ can be expressed as
\begin{align}\label{eq:recSig_final}
  &y_k = \overbrace{\sbrackets{\vecth_k^{\text{eff}}(\vectv)}^H \vectw_k^p s_k^p + \sum_{j \in \Phi_k} \sbrackets{\vecth_k^{\text{eff}}(\vectv)}^H \vectw_j^c s_j^c}^{\text{signals that are decoded}}+ \nonumber\\ &   \underbrace{\sum_{m \in \mathcal{K}\text{\textbackslash}\cbrackets{k}} \hspace{-0.35cm} \sbrackets{\vecth_k^{\text{eff}}(\vectv)}^H \vectw_m^p s_m^p \hspace{-0.05cm} +\hspace{-0.05cm} \sum_{\ell \in \Psi_k} \sbrackets{\vecth_k^{\text{eff}}(\vectv)}^H \vectw_\ell^c s_\ell^c + n_k}_{\text{interference plus noise}}.
\end{align}
Let ${\gamma_k^p}$ denote the \ac{SINR} of user $k$, decoding its private message, and let $\gamma_{i,k}^c$ denote the \ac{SINR} of user $i$, decoding the common message of user $k$. Let the vector $\vectw_k = \hbrackets{ \sbrackets{\vectw_k^p}^T , \sbrackets{\vectw_k^c}^T }^T \in \mathbb{C}^{2NL\times1}$ represent the stacked private and common beamformers of user $k$ and let the vector $\vectw = \hbrackets{ (\vectw_1)^T , (\vectw_2)^T , \dots , (\vectw_K)^T}^T \in \mathbb{C}^{2KNL\times1}$ represent all beamformers.\\
Using the partition in (\ref{eq:recSig_final}), $\gamma_k^p(\vectw,\vectv)$ and $\gamma_{i,k}^c(\vectw,\vectv)$ can be expressed as
\begin{align}
   &\gamma_k^p(\vectw,\vectv) = \label{eq:gammap}\\
   &\frac{|{\sbrackets{\vecth_k^{\text{eff}}(\vectv)}^H \vectw_k^p}|^2}
                     {\sum\limits_{m \in \mathcal{K}\text{\textbackslash}\cbrackets{k}} \hspace{-0.2cm} |{\sbrackets{\vecth_k^{\text{eff}}(\vectv)}|^H \vectw_m^p}^2 + \sum\limits_{\ell \in \Psi_k} |{\sbrackets{\vecth_k^{\text{eff}}(\vectv)}|^H \vectw_\ell^c}^2 + \sigma^2}, \nonumber\\
   &\gamma_{i,k}^c(\vectw,\vectv) = \label{eq:gammac} \\[-1pt] &\frac{|{\sbrackets{\vecth_i^{\text{eff}}(\vectv)}^H \vectw_k^c}|^2}
                     {T_i + \sum\limits_{\ell \in \Psi_i} |{\sbrackets{\vecth_i^{\text{eff}}(\vectv)}|^H \vectw_\ell^c}^2 +
                     \sum\limits_{m \in \Omega_{i,k}} |{\sbrackets{\vecth_i^{\text{eff}}(\vectv)}|^H \vectw_m^c}^2},\nonumber
   \vspace{-0.1cm}
\end{align}
where $T_i = \sum_{j \in \mathcal{K}}^{\phantom{I}} |\sbrackets{\vecth_i^{\text{eff}}(\vectv)}^H \vect{\omega}_j^p|^2  + \sigma^2$.
Furthermore, the sum-rate of the common and private rates can be defined, which has to be higher or equal than the \ac{QoS} $r_k^{\mathsf{Min}}$ of each user $k$, namely \vspace{-0.1cm}
\begin{align}
   R_k^p + R_k^c \geq r_k^{\mathsf{Min}},
\end{align}
where $R_k^p$ is the private rate and $R_k^c$ the common rate of user $k$.
The messages $s_k^p$ and $s_k^c$ are only decoded reliably if the private and common rates of each user satisfy the following conditions
\begin{align}\label{eq:privateRate}
 R_k^p &\leq   B \log_2 \big(1+\gamma_{k\phantom{.}}^p(\vectw,\vectv)\big)  , \quad \forall k \in \mathcal{K}\\
  R_k^c &\leq B \log_2 \sbrackets{1+\gamma_{i,k}^c(\vectw,\vectv) }, \quad  \forall k \in \mathcal{K} ,\, \forall i \in \mathcal{M}_k,\label{eq:commonRate}
\end{align}
where $B$ represents the transmission bandwidth. 



==> Publish5 v9 (conference-arxiv)/settings.tex <==
\usepackage{standard}
\usepackage{etex}
%\usepackage[commentsnumbered,ngerman,ruled,vlined,german]{algorithm2e}
\usepackage{rotate}
%\usepackage{booktabs}
%\usepackage{algorithmic}
\usepackage{algorithmic}
\usepackage{algorithm}
%\usepackage{algorithmic}
\usepackage{float}
\usepackage{tikz}
\usepackage{refcount}
\usepackage{caption}
\usepackage{pgf,tikz}
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\usepackage{bbm}
\usepackage{adjustbox}
\usetikzlibrary{calc}
\usepackage{relsize}
\usepackage{ifthen}
%\usepgfplotslibrary{external}
%\tikzexternalize
\usetikzlibrary{calc,fit,arrows,plotmarks,intersections,patterns,shapes,decorations,positioning, backgrounds, matrix}
%\tikzstyle{every picture}+=[remember picture]
\usepackage[numbers,sort&compress]{natbib}
%\bibliographystyle{dinat}
\usepackage[ngerman, english]{babel}
\usetikzlibrary{arrows.meta}
\edef\wdArrowLength{2}
\tikzset{>={Latex[width=1.5mm,length=\wdArrowLength mm]}}
\usepackage{graphicx}
\usepackage[outdir=./pictures]{epstopdf}
%%\tikzset{>=latex'}
%\pgfkeys{/pgf/number format/.cd,%
%	fixed,%
%		%fixed zerofill,%
%		%precision=2,%
%		set thousands separator={}}
%\pgfkeys{/pgf/number format/.cd,fixed,precision=1}
%\pgfdeclarelayer{myback}
%\pgfsetlayers{myback,background,main}
%
%\usepackage{verbatim}
%\usepackage{slashbox}
%%\usepackage{ngerman} %causes problems with babel
%\usepackage{array}
%\usepackage{etoolbox}
%\usepackage[british]{babel}
%\usepackage[commentsnumbered,ruled,vlined,german]{algorithm2e}
%\usepackage[T2A,T1]{fontenc}
%\usepackage[ansinew]{inputenc}
%\usepackage{ulem}
%\normalem
%%\usepackage{algpseudocode}
\usepackage{cancel}
%\usepackage{amsmath}
%\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{shadethm}
\usepackage[ansinew]{inputenc} % CHANGE HERE IF NECESSARY
\usepackage[T1]{fontenc}
%\newshadetheorem{sthm}{Definition}[section]
%\newtheorem{mysthm}{Definition}[section]
%\theoremstyle{definition}
%\newtheorem{dfn}{Definition}[section]
%\setbeamertemplate{theorems}[%ams style
%ams style
%]
\usepackage{empheq}
\usepackage{skull}
\usepgfplotslibrary{units}
\usepackage{calc}
\usepackage{nicefrac}
\usepackage{fancybox}
%\usepackage{pstricks, pst-text, pst-grad, pst-coil}
\usepackage{psfrag}
\usepackage{dsfont}
%\usepackage{subfig}
%\usepackage{breqn}
\newtheorem{prop}{Proposition}
\usepackage{pdfpages}
% Format page foot and header
\usepackage{scrlayer-scrpage}
%\clearscrheadings
%\clearscrheadfoot
%\automark[section]{chapter}
%\ofoot[\pagemark]{\pagemark}
%\ohead{\headmark}
\pagestyle{scrheadings}
\usepackage{hyphenat}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Set name and title % CHANGE HERE
\title{On Synergistic Benefits of Rate Splitting in IRS-assisted Cloud Radio Access Networks} % Title of the Thesis
\author{Kevin Weinberger, Alaa Alameer Ahmad, Aydin Sezgin\\ Ruhr-Universit\"at Bochum, Germany\\ Email:\{kevin.weinberger, alaa.alameerahmad, aydin.sezgin\}@rub.de,}
\date{\today}

% Set thesis type % CHANGE HERE
\newcommand{\thtype}{Master's}

% Load packages ...

% Figures
\usepackage{graphicx}
\usepackage{placeins}
%\usepackage{pstricks}

% Tables
\usepackage{booktabs}
\usepackage{marvosym}
\usepackage{multirow}

% Math stuff and units
\usepackage{latexsym, amsmath, amssymb, amsfonts, upgreek}
%\usepackage{siunitx}
\newcommand{\mathup}{\mathrm}

% Acronyms
\usepackage[nolist]{acronym}

% Enable quotes by \enquote{}
\usepackage[babel,english=american, german=quotes]{csquotes}

% Necessary for frontpage, allows to create automata and fancy graphics
\usepackage{tikz}
\usetikzlibrary{calc,arrows,positioning,decorations,shadows,shapes,fadings,matrix}
\tikzset{>=latex'}
\tikzset{semithick}

%%
%\renewcommand{\thealgorithm}{\arabic{chapter}.\arabic{algorithm}}
\makeatletter
\providecommand{\IfElsePackageLoaded}[3]{\@ifpackageloaded{#1}{#2}{#3}}
%
\makeatother

\usepackage{subfigure}
% Laden mit Option subfigure in Abhängigkeit vom Paket subfigure und subfig
\IfElsePackageLoaded{subfig}
	% IF subfig
	{\usepackage[subfigure]{tocloft}}{	
	% ELSE
	\IfElsePackageLoaded{subfigure}
		% IF subfigure
		{\usepackage[subfigure]{tocloft}}
	   % Else (No subfig nor subfigure)
		{\usepackage{tocloft}}
	}

%

%%

% Source code listings
\definecolor{colKeys}{rgb}{0,0,1}
\definecolor{colIdentifier}{rgb}{0,0,0}
\definecolor{colComments}{rgb}{1,0,0}
\definecolor{colString}{rgb}{0,0.5,0}

\usepackage{listings}
\lstset{%
    float=hbp,%
    basicstyle=\ttfamily\scriptsize, %
%    identifierstyle=\color{colIdentifier}, %
%    keywordstyle=\color{colKeys}, %
%    stringstyle=\color{colString}, %
%    commentstyle=\color{colComments}, %
    identifierstyle=\color{black}, %
    keywordstyle=\color{Blue}, %
    stringstyle=\color{Green}, %
    commentstyle=\color{Gray}, %
    columns=flexible, %
    tabsize=2, %
    frame=single, %
    extendedchars=true, %
    showspaces=false, %
    showstringspaces=false, %
    numberstyle=\tiny, %
    breaklines=true, %
    backgroundcolor=, %
    breakautoindent=true, %
	language=Matlab,
	numbers=left,
	emph={block},
	emphstyle={\color{Red}},
    captionpos=b%
}
% TikZ nodes
\tikzstyle{dot} = [draw, circle, minimum size=0.2pt, scale=0.3, fill=black]
\tikzstyle{state} = [draw, circle, minimum width=1cm]
\tikzstyle{myloop} = [->,to path={.. controls +(45:1) and +(135:1) .. (\tikztotarget) \tikztonodes}]
\tikzstyle{block} = [draw, fill=blue!20, rectangle, rounded corners, drop shadow, minimum height=3em, minimum width=6em]
\tikzstyle{pc-or} = [draw, fill=blue!20, rectangle, rounded corners, drop shadow, minimum height=6em, minimum width=5em]
\tikzstyle{scan-or} = [draw, fill=red!80, rectangle, rounded corners, drop shadow, minimum height=6em, minimum width=5em]
%\tikzstyle{snakeline} = [decorate, decoration={pre length=0.2cm, post length=0.2cm, snake, amplitude=1mm, segment length=3mm},very thin]
\tikzstyle{dot2} = [draw, circle, minimum size=0.2pt,scale=0.3,fill=black,black]
\tikzstyle{ant} = [regular polygon,regular polygon sides=3, draw,shape border rotate=180,minimum size=0.2pt,scale=0.3]
\tikzstyle{connector} = [->,thick]
\tikzstyle{snakeline} = [connector, decorate, decoration={pre length=0.2cm, post length=0.2cm, snake, amplitude=.4mm, segment length=2mm}]

\newcommand{\myant}[2]{ % args: label, position
\node (#1) at (#2) [inner sep=2.5pt] {};
\draw (#1.west) to (#1.south);
\draw (#1.east) to (#1.south);
}

% Algorithms
%%\usepackage[ruled, vlined, linesnumbered,algosection,algo2e]{algorithm2e}
%\usepackage{algorithmic}
%\usepackage[chapter]{algorithm}

% pgfplots
\usepackage{pgfplots}
\usepackage{pgfplotstable}
%\usepgfplotslibrary{units}
%\pgfplotsset{compat=1.4}
\usetikzlibrary{spy}



% Format page foot and header
\usepackage{scrlayer-scrpage}
%\clearscrheadings
%\clearscrheadfoot
%\automark[section]{chapter}
\ofoot{\pagemark}
\ohead{\headmark}
\pagestyle{scrheadings}

%% use some standards for mathematical expressions:
\newcommand{\red}{{\rm red}}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{definition}[theorem]{Definition}
%\newtheorem{algorithm}[theorem]{Algorithm}
\newtheorem{example}{Example}[chapter]
%\newenvironment{example}{\begin{quote}{\bf Example:}}{\end{quote}}
%\newenvironment{example}{{\bf Example:}}{}



% BIBTEX, http://merkel.zoneo.net/Latex/natbib.php
% if you uncomment this block, you'll get an english bibliography with alphanumerical references
%\usepackage{bibgerm} % u. a. statt et al
%\usepackage[square,numbers]{natbib} % eckige klammern, natbib-package
% \setbibpreamble{{\large Seitenzahlen, auf denen ein Eintrag referenziert wird, werden am Ende eines jeden Eintrags angegeben.}\newline} % Wegen der pagebackref-Option des hyperref-Packets, wird vielen nicht direkt klar was das soll http://projekte.dante.de/DanteFAQ/Verzeichnisse#16

%\bibliographystyle{dinat} % deutsches lit-verz: Diplomarbeit, Seite x-y, ...
%\bibliographystyle{alpha}

% gray definition boxes, that whay you'll find them in the text
\usepackage{shadethm}
\newshadetheorem{sthm}{Definition}[chapter]
\newenvironment{definition}[1][]{
   \definecolor{shadethmcolor}{rgb}{.9,.9,.9}
   \begin{sthm}[#1]
 }{\end{sthm}}

% light gray example boxes,
%\newshadetheorem{sthmex}{Example}[chapter]
%\newenvironment{example}[1]{
%   %\definecolor{shadethmcolor}{rgb}{.99,.99,.99}
%   \begin{sthmex}[\text{#1}]
% }{\end{sthmex}}


% experimental
%\usepackage{scrhack}

% Hyperlinks and menu for your document
\usepackage[breaklinks,hyperindex,colorlinks,anchorcolor=black,citecolor=black,filecolor=black,linkcolor=black,menucolor=black,urlcolor=black,pdftex]{hyperref} % pagebackref: Add page number to the references where they can be found
\usepackage{breakurl}

\makeatletter
\AtBeginDocument{
 \hypersetup{
   pdftitle = {\@title},
   pdfauthor = {\@author},
   pdfsubject={\@title},
   pdfkeywords={Generating Secure Cryptographic Keys Channel Properties Matlab Simulink}, % CHANGE HERE
%    unicode={true},
 }
}

%% TikZ: Underbraces
\def\tikz@delimiter#1#2#3#4#5#6#7#8{%
	\bgroup
		\pgfextra{\let\tikz@save@last@fig@name=\tikz@last@fig@name}%
		node[outer sep=0pt,inner sep=0pt,draw=none,fill=none,anchor=#1,at=(\tikz@last@fig@name.#2),#3]
		{%
			{\nullfont\pgf@process{\pgfpointdiff{\pgfpointanchor{\tikz@last@fig@name}{#4}}{\pgfpointanchor{\tikz@last@fig@name}{#5}}}}%
			\delimitershortfall\z@% as suggested by morbusg (maximum space not covered by a delimiter = 0)
			\resizebox*{!}{#8}{$\left#6\vcenter{\hrule height .5#8 depth .5#8 width0pt}\right#7$}%
		}
		\pgfextra{\global\let\tikz@last@fig@name=\tikz@save@last@fig@name}%
	\egroup%
}




==> sections/preliminaries.tex <==
\section{Power Minimization Techniques}\label{ch:PowMin}
\input{sections/preliminaries/rate_splitting.tex}
\input{sections/preliminaries/intelligent_reflective_surface}


==> sections/preliminaries/intelligent_reflective_surface.tex <==
\subsection{Intelligent Reflecting Surface}
Since the beginning of wireless communication networks, the medium between the transmitter and receiver has been modeled as a randomly behaving entity. The randomness of the surroundings, which the transmitted radio waves are subjected to and uncontrollably interacting with, causes the quality of received signal to degrade.\\
Intelligent reflecting surfaces, also known as Large Intelligent Surfaces, Intelligent Reconfigurable Surfaces, Software-controlled Metasurfaces and more, comprise an array of reflect elements, that are able to influence, and consequently control the \nohyphens{reflection} of the incident signal. The change of the reflected signal may be about the amplitude, phase, frequency and polarization \cite{IRSTheoPerfLim}. As each reflect element can be independently controlled by a smart controller, the IRS is able control the wireless propagation environment to establish favourable channel responses. Therefore, the IRS is able to generate controllable passive beamforming as depicted in Figure \ref{fig:IRSsimple}.\\
\\
The \ac{IRS} and its controllable reflect elements can be modeled as depicted in Figure \ref{fig:IRSModel}, where an IRS consisting of $R$ reflect elements is considered. The figure shows that each antenna of the transmitter has a channel $h_r$ to each reflect element of the IRS and a direct channel $h_0$ to the user. At the IRS, the induced changes on the incident signal caused by $r$-th reflect element are captured with the reflection coefficient $v_r$. After inducing the changes, each reflect element reflects the signal to the receiver through a channel $g_r$. It is noted that the channels $g_r$ from the IRS to the receiver differ from the channels $h_r$ between the IRS and the transmitter. The change of amplitude $\beta_r$ and phase $e^{j\theta_r}$ on the reflected signal caused by the $r$-th reflect element could therefore be represented by defining its reflection coefficient as $v_r = \beta_r e^{j\theta_r}$ .\\
\begin{figure}
\centering
\includegraphics[width=\columnwidth]{pictures/IRS_simple}
\caption{Intelligent Reflecting Surface (\ac{IRS})}
\label{fig:IRSsimple}
\end{figure}
\begin{figure}
\centering
\includegraphics[width=\columnwidth]{pictures/IRS-modell}
\caption{Model of an intelligent reflecting surface with $R$ reflect elements, where $h_0$ represents the channel of the direct \ac{LoS} path between transmitter and receiver and $v_r$ represents the reflect coefficient of the $r$-th element.}
\label{fig:IRSModel}
\end{figure}
The first concept of a reflecting surface in wireless communication systems dates back to 1963, in which the reflecting elements of a \textit{Reflectarray}  were mounted directly to the antenna in order to generate different radiation patterns \cite{ReflectArray}. Recent advancements, however, made it possible to reconfigure the changes on the incident signal in real time \cite{IRSrealtimeChange1,IRSrealtimeChange2},
which made the use of \ac{IRS}s applicable in modern wireless communication systems \cite{AnasIRSImprovement,IRSImprovement1,IRS_EEvsRelay,AnasIRSAnalysis}. In recent works, the changes induced to the incident signal by the \ac{IRS} are assumed to be phase shifts \cite{IRS_EEvsRelay,IRS_MIMO+Transmission}, which implies that the \ac{IRS} is passive in its ideal form, and therefore does not consume any of the available transmit power. However, since the phase shifts, that the \ac{IRS} induces, need to be adjusted regularly in order to positively impact the changing transmission scenarios, the \ac{IRS} requires a control signal, and consequently active components like the smart controller for adaptive phase shifting.\\
By correctly aligning its phase shifts, the \ac{IRS} is able to superposition phase shifts at the receiver to achieve either constructive interference to improve data rates or destructive interference to remove interference \cite{AnasIRSImprovement,IRSImprovement1,IRS_EEvsRelay}. The latter is also useful for enhancing security and privacy, which can be achieved by improving the physical layer security as the reflected signals can be configured to cancel out the \ac{BS}-to-eavesdropper \ac{LoS} signals. This effectively reduces the information leakage \cite{IRSpositioning}.\\ \\
Contrary to the first concept, \ac{IRS}s can be easily deployed on walls, buildings and ceilings of any shape, indoors and outdoors \cite{IRS_MIMO+Pos} because they can be practically fabricated to any arbitrary shaped surface, due to the modularity of the reflect elements \cite{IRSpositioning}. Moreover, the extension of any wireless network with \ac{IRS}s can be done without any major modification in the hardware and software of user equipment because the users effectively benefit from amplified channels.\\
\\
For obtaining an optimal transmission environment, the transmitter needs to be able to send a control signal to the \ac{IRS}. In recent works \cite{AnasIRSAnalysis,IRSImprovement1,IRScontroller,IRScontrollerII}, which study single-cell \ac{IRS}-assisted scenarios, a fronthaul link is employed, that connects the transmitter to a smart controller, which tunes the \ac{IRS} reflect elements based on the received signal. Because of the \ac{IRS}-assisted \ac{C-RAN} employed in this work, the central processor of the cloud is able to assume the tasks of the smart controller.\\
\\
%Figure \ref{fig:IRS-CRAN} depicts a simple \ac{IRS}-assisted \ac{C-RAN} transmission scenario with two users and two base stations, where the central processor of the cloud manages the control signal for the \ac{IRS} adjustments. The cloud also distributes the requested messages to the base stations, which then transmit the signals in the \ac{IRS}-enhanced environment. It is noted, that the \ac{IRS} reflects the transmit signals of each base station in reach to each user in reach. Hence, the reflected signal, that each user receives, can carry a desired and undesired part for the respective user and thus can either improve or deteriorate the users signal to interference and noise ratios, based on the current \ac{IRS} setting. Therefore, finding the optimal setting for the reflect elements of the \ac{IRS} is a crucial task for the improvement of  \ac{IRS}-assisted transmission scenarios. \\
Due to the similarities to relays in forwarding received signals, the performance of \ac{IRS}s can be compared to the performance of relays \cite{AnasIRSAnalysis,RelayIntelligentRS,bjornsonIRS}. In \cite{bjornsonIRS} it was shown that while decode-and-forward (DF) relaying suffers from pre-log penalty due to the two-hop transmission, the reflections from the \ac{IRS} must travel over two channels, from the transmitter to the \ac{IRS} and from the \ac{IRS} to the receiver, to reach the destination. This leads to a very small channel gain per reflect element of the \ac{IRS}. To meet the performance of the relay, many reflect elements have to be employed in order to counteract the low channel gain. However, even with hundreds of elements, the \ac{IRS} can still be of relatively small size because each reflect element is assumed to have a sub-wavelength size \cite{smallSize1,smallSize2} and can still remain cost-effective because the production cost of the reflect elements is low. Contrary to relays, there are no power amplifiers needed for the \ac{IRS} in its ideal form, which also means that there is no new interference introduced when using \acp{IRS} to improve the transmission scenario. Moreover, it has been shown that \acp{IRS} are able to significantly decrease network power consumption \cite{IRS_powerconsumpt} if deployed to aid wireless communication systems. Therefore, an \ac{IRS} can be more energy efficient than regular multi-antenna amplify-and-forward relaying \cite{IRS_EEvsRelay,bjornsonIRS}. However, even if deploying an \ac{IRS} is not the most efficient or effective solution, the low cost and versatility regarding deployment locations still makes the \ac{IRS} a viable alternative.\\
Another challenge that arises with the use of \acp{IRS} in communication systems is the need for new communication-theoretic models \cite{newComTheoModels}. In fact, in current wireless networks the devices and transmission protocols are designed to adapt themselves to the current transmission scenario. In this case, the devices are the endpoints of the communication environment, which is treated as unintentional and uncertain interference to the transmission. Incorporating an \ac{IRS} to the communication scenario adds another degree of freedom to the transmission scenario and enables the environment to behave smartly \cite{newComTheoModels}.
%Hence, instead of optimizing only the endpoints, i.e transmitter and receiver, Smart Radio Environments can be configured dynamically and support the transmission scenario \cite{newComTheoModels}.


==> sections/preliminaries/rate_splitting.tex <==
\subsection{Rate Splitting and Common Message Decoding}
Delivering different types of messages to different types of users has been of great interest with the emerging technologies and appliances of \ac{IoT}. Furthermore, with the deployment of more devices into small cells, the distances between the users and \acp{BS} decreases. As a consequence, the direct \ac{LoS} channels become stronger and of better quality to the detriment of increasing inter-BS interference because of close proximity of \acp{BS} in neighbouring cells. For conventional transmission schemes, which use treating interference as noise as strategy, these changes to the transmission scenario degrade the overall network performance significantly, especially in already interference-limited dense networks \cite{aydin-sub-opt,aydin-crystal}.\\
\\
In contrast to \ac{TIN}, the \ac{RS-CMD} strategy for the two-user \ac{IC} consists of splitting the messages of each user into two parts, a private part, that is decoded by the intended user only, and a common part, that can be decoded at both, the intended user as well as the interfered user in the network  \cite{RS-Base}. This scenario is depicted in Figure \ref{fig:RSsimple}, where each \ac{BS} splits the message of its allocated user into a common and private part. The figure shows that user $1$ receives the private and common messages of both users. However, user $1$ is able to decode the common message $\hat{s}_2^c$ of user $2$ before decoding its own common and private message $\hat{s}_1^c$ and $\hat{s}_1^p$. The ability to decode the common message of other users enables both users to cancel out a part of their received interference. Figure \ref{fig:RSsimple2} shows the \ac{SIC} receiver at user $1$, which enables mitigating the interference caused by the common message $\hat{s}_2^c$ of user $2$ by applying \ac{SIC}. Therefore, using the \ac{RS-CMD} strategy can increase the achievable data rates when compared to the TIN strategy. In fact, for the two-user \ac{IC} it has been shown, that the \ac{TIN} strategy is suboptimal \citep{RS-Base,Kobayashi,WithinOneBit,CapacityAydin}, while the \ac{RS-CMD} strategy has been shown to approach the largest capacity region of the \ac{IC} to within one bit \cite{Kobayashi,WithinOneBit}.
\begin{figure}
\centering
   \includegraphics[scale=0.9]{pictures/rate-splitting_simple_nc}
   \caption{\ac{RS-CMD} strategy for the two-user IC. Each \ac{BS} splits the message of its allocated user into a private and common part.}
\label{fig:RSsimple}
\end{figure}
\begin{figure}
\centering
   \includegraphics[scale=1.1]{pictures/rate-splitting_simple_nc2}
   \caption{Successive Interference Cancellation Receiver at User 1}
\label{fig:RSsimple2}
\end{figure}
The idea of splitting the messages of each user with the intent to mitigate interference can be extended to a scenario with multiple users, in which the common parts are decoded by a selected group of receivers with the aim of mitigating interference within this group. To ensure that each user in this group is able to decode the same common message, the achievable common rate of each user in this group, decoding the common message of this group, has to be equal. For this reason, finding suitable groups of users, which decode the same common messages, is an important task for determining the gain of \ac{RS-CMD} over \ac{TIN} \cite{AlaaRSCMD}. Furthermore, more layers of the successive decoding strategy at the receivers can be employed \cite{AlaaRS,AlaaRSCMD}, which improves the performance of \ac{RS-CMD} for dense networks, in which each receiver is subjected to multiple sources of interference. Hence, \ac{RS-CMD} provides a high flexibility with regards to the allocation of rates, beamforming design and range of decoding layers and can provide a significant improvement in performance, especially in dense networks. In fact, it has been shown that rate splitting is a generalization of classical linear precoding methods and is able to improve the spectral efficiency in downlink broadcast channels considerably \cite{gen_linprecoder}. Moreover, applying  \ac{RS-CMD} beyond the two-user interference channel to a multi-cell multiuser downlink scenario, subject to minimum achievable rate constraints across the users, has been shown to bring substantial benefit in terms of improving the maximum minimal rate, especially for cell-edge users as they are able to mitigate inter-cell interference \cite{RS-Theo2Prax}.\\
\\
However, in rate splitting, the cooperation of multiple \acp{BS} is required in order to deliver the private and common messages to the users because the messages have to be split and encoded jointly. In fact, the transmitted signals at the \acp{BS} are designed as superpositions of the private and common messages. Therefore, a suitable platform for the physical implementation of rate splitting techniques is the \ac{C-RAN} architecture, which is able to virtualize baseband functionalities to a centralized cloud entity. This central processor (\ac{CP}) is connected to the \acp{BS} in the cloud-enabled network and facilitates centralized processing, that can be utilized to apply enhanced interference management techniques, which are superior to classical interference management techniques in \ac{MIMO} networks \cite{MIMO-CRAN-interference-mitigation,AlaaRS,AlaaRSCMD}. Due to this hierarchy, the \ac{CP} is able to jointly encode the messages for each user and design the transmit signals for cooperating clusters of \acp{BS}, subject to per-user \ac{QoS} constraints, with the aim to maximize the interference mitigation effects. It has been shown that using \ac{RS-CMD} in combination with the \ac{C-RAN} architecture, in order to mitigate interference, provides a significant gain if compared to interference mitigation techniques, that do not rely on \ac{RS-CMD} \cite{AlaaRSCMD}. In fact, it has been shown that the use of \ac{RS-CMD} in \ac{MIMO} \ac{C-RAN} systems can achieve gains of up to 97\% in terms of the energy efficiency \cite{Alaa_EE_RSCMD} and 27\% in terms of the achievable maximum sum-rate \cite{Alaa_27} over the baseline scheme of treating interference as noise.



